Explingo: Explaining AI Predictions using Large Language Models

Explanations of machine learning (ML) model predictions generated by Explainable AI (XAI) techniques such as SHAP are essential for people using ML outputs for decision-making. We explore the potential of Large Language Models (LLMs) to transform these explanations into human-readable, narrative formats that align with natural communication. We address two key research questions: (1) Can LLMs reliably transform traditional explanations into high-quality narratives? and (2) How can we effectively evaluate the quality of narrative explanations? To answer these questions, we introduce Explingo, which consists of two LLM-based subsystems, a Narrator and Grader. The Narrator takes in ML explanations and transforms them into natural-language descriptions. The Grader scores these narratives on a set of metrics including accuracy, completeness, fluency, and conciseness. Our experiments demonstrate that LLMs can generate high-quality narratives that achieve high scores across all metrics, particularly when guided by a small number of human-labeled and bootstrapped examples. We also identified areas that remain challenging, in particular for effectively scoring narratives in complex domains. The findings from this work have been integrated into an open-source tool that makes narrative explanations available for further applications.

==> CHI2024_workshop/conclusions.tex <==
\label{sec:conclusions}
In this paper, we have laid the groundwork for exploring the use of LLMs in XAI by focusing on transforming ML explanations into natural, human-readable narratives. 
By establishing metrics for evaluating narrative explanations and experimenting with prompt-design, we demonstrated the ability of LLMs, particularly GPT-4, to generate sound, complete, and context-aware explanation narratives.

%Our initial experiments involved applying prompt tuning techniques with GPT-3.5 and GPT-4 on two datasets. 
%So far, we have defined metrics 
%such as accuracy, completeness, context-awareness, fluency, and response length 
%to evaluate generated narrative explanations, and employed these in a prompt-tuning experiment. Results indicate GPT-4's superiority in accuracy, completeness, and context-awareness over GPT-3.5. %, while GPT-3.5 performed better in fluency and produced shorter answers.
%We then conducted a pilot user study to measure user perception of narrative-based explanations compared to traditional XAI visualizations. 
Our pilot user study found that a majority of participants favored narrative-based explanations, finding them easier to understand and more informative. This provides promising insights into the potential benefits of adopting LLM-based narrative explanations.

Moving forward, we aim to further investigate the proposed research directions, such as %. Future work will 
using fine-tuning methods, trying additional LLMs, and exploring the integration of training data and external guides to create context-aware explanations. Future work will also include a larger user study for a more comprehensive evaluation of narrative-based explanations compared to traditional methods.

%Our findings of this study suggest concrete takeaways for the advancement of XAI. 
We offer the following concrete takeaways for the advancement of XAI.
First, the adoption of LLM-based narrative explanations can lead to enhanced user understanding of ML outputs. Second, the superior performance of GPT-4 underscores the advancements in LLM capabilities and their potential impact on XAI. Finally, there remain many promising directions for future research to enhance the quality of narrative explanations.
%the promising future directions identified highlight avenues for further research to enhance context-awareness in narrative explanations.


%Moreover, an in-depth user study with a larger participant pool will be conducted to validate and generalize our initial findings.

%In conclusion, this study sets the stage for a comprehensive exploration of LLMs in the context of XAI, with a specific focus on natural, human-readable narrative explanations. 
%To conclude, the proposed research provide contributions to the ongoing trend of making AI systems more transparent, interpretable, and usable.


Ultimately, our research contributes to the ongoing trend of making AI systems more transparent, interpretable, and usable. By providing users with narrative-based explanations, we aim to foster trust and understanding in AI technologies, thereby promoting their responsible and ethical use in diverse domains.

==> CHI2024_workshop/exp_setup.tex <==
\newcommand{\accuracy}{soundness}
\newcommand{\fluency}{fluency}
\newcommand{\completeness}{completeness}
\newcommand{\contextawareness}{context-awareness}
\newcommand{\Accuracy}{Soundness}
\newcommand{\Fluency}{Fluency}
\newcommand{\Completeness}{Completeness}
\newcommand{\Contextawareness}{Context-awareness}


\section{Research Directions}
Here we list several directions to investigate and improve LLMs for generating explanation narratives.

\textbf{R1. Defining evaluation metrics: } To allow researchers to compare narrative explanations from different models and techniques, formal metrics for evaluation must be defined.
%Before research can be done on narrative explanations, formal metrics for evaluation must be defined. 
Existing work \cite{xieInterpretationQualityScore2022a, zhouEvaluatingQualityMachine2021} proposes metrics for evaluating XAI explanations in general; in this paper, we propose an initial set of metrics adapted specifically for LLM-generated natural-language explanations. %models and prompts.

\textbf{R2. Prompt Design:} 
It is worth investigating how well LLMs are able to generate explanation narratives in a zero-shot manner. 
Prompt design involves crafting specific prompts to guide language models in producing nuanced and contextually varied explanations. This contributes to the robustness of the evaluation by mitigating the potential bias introduced by a single prompt. In this paper, we try five prompts on pretrained LLMs (particularly, GPT-3.5 and GPT-4).

\newcounter{PCounter}
\newcommand{\PLabel}[1]{%
    \refstepcounter{PCounter}% Increment the counter
    \label{#1}
    P\thePCounter% Print the label
}

\begin{table*}[t!]
\footnotesize
\caption{The prompts used for our initial experiments. Recurring components are at the top, followed by the five prompts. The context description in [INTRO] and the values in [EXP] varied by dataset and input. P\ref{prompt:fluent} and P\ref{prompt:context} were designed to address shortcomings in responses from P\ref{prompt:basic} (a lack of \fluency{} or \contextawareness{} respectively). P\ref{prompt:novals} and P\ref{prompt:vals} show examples of fulfilling specific user needs through prompt tuning.} 
\begin{tabular}{cp{0.9\textwidth}}
\toprule
\textbf{Code} &
  \textbf{Recurring Component} \\ \midrule
  {[}INTRO{]} &
   You are helping users understand an ML model's prediction. The model predicts house prices. \\ \addlinespace
{[}TASK{]} &
  I will give you feature contribution explanations, generated using SHAP, in (feature, feature\_value, contribution, average\_feature\_value) format. Convert the explanations in simple narratives. Do not use more tokens than necessary. \\ \addlinespace
 {[}EXP{]} & (Second floor square feet, 854, 12757.83, 583.0), (Construction date, 2003, 9115.72, 1976.1), (Basement area in sq. ft., 856, -6157.86, 1073.6) \\ \midrule
\textbf{Code} &
  \textbf{Prompt} \\ \midrule
\PLabel{prompt:basic} &
  {[}INTRO{]}{[}TASK{]}{[}EXP{]} \\ \addlinespace
\PLabel{prompt:fluent} &
  You are helping users who do not have experience working with ML understand an ML model's predictions. {[}TASK{]}. Make your answers sound as natural as possible, as though said in conversation. {[}EXP{]} \\ \addlinespace
\PLabel{prompt:context} &
  {[}INTRO{]}{[}TASK{]} Include context on how the specific instance compares to the average, and ensure the explanation highlights the significance of each feature's contribution to the overall prediction. {[}EXP{]}  \\ \addlinespace 
\PLabel{prompt:novals} &
  {[}INTRO{]}{[}TASK{]} Do not explicitly mention any feature or contribution values in your response. {[}EXP{]} \\ \addlinespace
\PLabel{prompt:vals} &
  {[}INTRO{]}{[}TASK{]} Be sure to explicitly mention all feature and contribution values in your response. {[}EXP{]} \\ \bottomrule  
\end{tabular}
\label{tab:prompts}
\end{table*}

% \begin{table*}[ht]
%     \centering
%     \begin{tabular}{|c|p{0.9\textwidth}|}
%         \hline
%         \textbf{Code} & \textbf{Prompt} \\
%         P1 & [intro] [task]. Convert the explanations in simple narratives. Do not use more tokens than necessary.\\
%         P2 & You are helping users who do not have experience working with ML understand an ML model's predictions. [task]. Convert the explanations in simple narratives. Do not use more tokens than necessary. Make your answers sound as natural as possible, as though said in conversation. \\
%         P3 & [intro] [task] Convert the explanations in simple narratives. Do not use more tokens than necessary. Do not explicitly mention any feature or contribution values in your response. \\
%         P4 & [intro] [task] Convert the explanations in simple narratives. Do not use more tokens than necessary. Be sure to explicitly mention all feature and contribution values in your response. \\
%         P5 & [intro] [task] Convert the explanations in simple narratives. Do not use more tokens than necessary. Include context on how the specific instance compares to the average, and ensure the explanation highlights the significance of each feature's contribution to the overall prediction. \\
%         \hline
%     \end{tabular}%
%     \caption{}
%     \label{tab:prompts}
% \end{table*}

\begin{table*}[ht]
    \centering
        \caption{Metrics used to rate explanations. As indicated by arrows, for \accuracy{}, \fluency{}, and \contextawareness{}, we assume higher values are better. For length, lower values are better. For \completeness{}, a score of 1 or 2 may be preferred depending on the target audience.}
    \resizebox{0.97\textwidth}{!}{%
    \begin{tabular}{|p{0.3\textwidth}|p{0.32\textwidth}|p{0.32\textwidth}|p{0.3\textwidth}|}
        \hline
        \textbf{Metric} & \textbf{0} & \textbf{1} & \textbf{2} \\
        \hline
        \textbf{\Accuracy{} \textuparrow :} The correctness of the information included in the narrative.  &
        The narrative includes one or more objective errors, such as reporting an incorrect contribution. & The narrative includes one or more misleading statements. For example, referring to a rating of 5 out of 10 as ``high''. & The narrative contains no errors. \\
        \hline
        \textbf{\Fluency{} \textuparrow :} The extent to which the narrative sounds ``natural'' or like it was generated by a human peer in conversation. & The narrative is very unnatural or confusingly worded, or directly repeats the given feature names and values without any narrative flow. & The narrative is somewhat natural. & The narrative sounds very natural, as though written by a human peer with good language skills. \\
        \hline
        \textbf{\Completeness{} \textendash :} The amount of information included in the narrative. & Some features given were missed entirely, or the direction of their contributions was not specified. & All features were described, but exact feature or contribution values were not given. & All feature values are given, and all contributions are described with directions and either exact values or descriptions (``contributed slightly''). \\
        \hline
        \textbf{\Contextawareness{} \textuparrow :} The degree to which the narrative ``explains the explanation'' by providing external context. & No context information is provided. & The answer includes references and comparisons to the average/mode feature values. & The answer includes further explanations of what may cause a specific contribution. \\
        \hline
        \textbf{Length} \textdownarrow & \multicolumn{3}{|p{0.9\textwidth}|}{The number of words in the response.} \\
        \hline
        
    \end{tabular}%
    }
    \label{tab:explanation_metrics}
\end{table*}


\textbf{R3. Comparing LLMs:}
Burton et. al. \cite{burton2023natural} demonstrated the effectiveness of smaller language models (T5 and BART) in generating explanation narratives. A thorough analysis comparing the effectiveness of newer, larger models in generating explanation narratives will contribute to a deeper understanding of their strengths and weaknesses.

\textbf{R4. Further training and finetuning:}
Explanation narratives generated by LLMs can be improved through the use of training methods such as model finetuning. For example, Burton et. al. \cite{burton2023natural} employed eight computer scientists to create a dataset of narrative versions of ML explanations. We propose furthering this work through a similar dataset generated by a larger group of non-technical experts, who may generate more broadly applicable samples.
%the use of a crowd-generated ``explanation dataset'' that converts ML explanations to readable narratives that can be used to improve the generated narratives. 

\textbf{R5. Integration of Training and Other External Data:}
Information from the model's training data, as well as other external information about the domain such as guides or textbooks, can be integrated into the explanation generation process to get more context-aware explanations using techniques such as Retrieval-Augmented Generation (RAG). Guo et. al. \cite{guoAdaptingPromptFewshot2023} demonstrated the effectiveness of this approach for generating natural-language descriptions of tables; extending this concept to ML explanations may contribute to more comprehensive narratives.

%\textbf{R6. Interactivity:}
%A benefit of LLMs is their ability to answer questions and smoothly interact with users, beyond just providing a single explanation. Works such as \cite{nguyen2023black}, \cite{shenConvXAIDeliveringHeterogeneous2023}, and  \cite{slack2023explaining} have introduced conversational agents to XAI using LLMs; coupling this with LLMs furthered tuned to create fluent and useful explanations will further the benefit of such agents.

We hope these directions provide a roadmap for further investigation into using LLMs for XAI. In the next section we introduce our current progress in some of these directions.


\section{LLMs for XAI: First Steps}

\label{sec:experimental_setup}
We began by investigating how well LLMs can transform explanations into narratives in a zero-shot manner, without any additional training, using GPT-3.5 and GPT-4. To begin with, we are focusing on SHAP explanations as inputs.

We applied a technique called prompt design, or crafting prompts to guide the language models in producing accurate and useful explanations. At this time, we have experimented with five prompts, shown in Table \ref{tab:prompts} (\textbf{R2}). 

To empirically compare the results from different prompts and models (and in the future, additional training methods), we adapted the metrics summarized by Zhou et. al. \cite{zhouEvaluatingQualityMachine2021} to evaluate XAI explanations (\textbf{R1}). As proposed in this work, we use the metrics of \textit{\completeness{}} and \textit{\accuracy{}} to measure the degree to which the narrative accurately represents the original explanation. We replace the term clarity with the more natural-language-specific term \textit{\fluency{}}, and use a simple \textit{length} metric to rate the parsimony of explanations. We also add an additional metric we call \textit{\contextawareness{}}, which considers the unique ability of LLMs to include additional contextual information ``explaining explanations'', beyond that provided by the base explanation.

Our five resulting metrics are described in Table \ref{tab:explanation_metrics}, and are scored on a scale from 0 to 2 (except length). We note that metrics such as \fluency{} are subjective and should be scored by multiple judges. For the work-in-progress experiments described in this paper, the authors rated the responses themselves. 


\subsection{Prompt Design Initial Results}
We conducted experiments on two datasets: the student performance dataset \cite{cortez_using_2008} and the Ames housing dataset \cite{de_cock_ames_2011}. We generated SHAP explanations on three instances (input rows) from each dataset, and selected the top three most contributing features as input to the LLM. We then combined these inputs with our five prompts, asking the LLM to generate readable narratives with different parameters\footnote{Details on our experimentation and results can be found at: https://github.com/sibyl-dev/Explingo}. For each of our two test models (GPT-3.5 and GPT-4), we generated and evaluated 90 explanation narratives (5 prompts $\times{}$ 2 datasets $\times{}$ 3 instances $\times{}$ 3 distinct responses). Table~\ref{tab:metric-results} shows the average scores obtained for each model across all the prompts.

%We generated and evaluated three distinct explanations per dataset, model, and prompt. This process was repeated on more than one explanation to ensure a robust set of generated explanations for subsequent evaluation.

GPT-3.5 gives shorter and more fluent responses than GPT-4. GPT-4 performs better on \accuracy{}, \completeness{} and \contextawareness{}. Notably, GPT-4.0's explanations included few errors; however, in real-world high-stakes decision-making contexts, we believe \accuracy{} would need to be consistently scored at 2.

%GPT-4 performs better than GPT-3.5 on \accuracy{}, \completeness{} and \contextawareness{}. However, GPT-3.5 performs better on \fluency{}, and gives shorter responses. Notably, GPT-4 exhibits a relatively higher \accuracy{} score; however, in high-stakes decision-making contexts, we believe \accuracy{} needs to be closer to 2 for real-world deployment.

\begin{table}[t]
\caption{Average ratings on our metrics across all prompts.} \label{tab:metric-results}
\centering
\resizebox{\linewidth}{!}{\begin{tabular}{lccccc}
\toprule
\textbf{Model} & \textbf{\Accuracy{}} & \textbf{\Fluency{}} & \textbf{\Completeness{}} & \begin{tabular}{@{}c@{}}\textbf{Context-} \\ \textbf{Awareness}\end{tabular} & \textbf{Length} \\
\midrule
GPT-3.5 & 1.211 & 0.811 & 1.422 & 0.522 & 380.611 \\
GPT-4  & 1.789 & 0.778 & 1.700 & 0.889 & 793.122 \\
\bottomrule
\end{tabular}}
\end{table}

\subsection{User Study}
To understand how people perceive narrative-based explanations versus traditional explanations, we ran a pilot user study. We recruited 20 participants from a random global pool through Prolific\footnote{https://www.prolific.com/}.
%This is an initial step into a thorough investigation into the use of LLM-based explanations for decision-making.

We selected the best-rated narrative explanations from our prompt design experiment and generated corresponding bar graph visualizations, resulting in two explanation types (narrative and plot-based). %
%Figure \ref{} shows an example of a bar-plot/narrative explanation pairing.
Each participant was shown 12 explanations (2 datasets $\times{}$ 3 instances $\times{}$ 2 types). For each explanation, we asked six subjective questions about the user's reception of the explanation, answered on a five-point Likert-type scale. The questions selected were inspired by existing literature for rating explanations and systems \cite{brooke1996sus, hoffman_measures_2023}, specifically chosen to relate to the perceived usability or clarity of explanations. Table \ref{tab:user-study-summary} summarizes the responses to these questions. 

At the end of the study, we asked participants to compare the two explanation types overall. Twelve participants reported preferring narrative-based explanations overall, compared to four for plot-based explanations (the remaining reported no preference). Eleven participants found narrative-based explanations easier to understand compared to five for plot-based, and twelve found narrative-based explanations more informative, compared to six for plot-based.

Overall, our findings motivate the potential benefits of an effective method for generating narrative explanations.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[t]
\centering
\caption{Summary of results from user study. Each rating is converted as strongly disagree=1, strongly agree=5, and then averaged. Narrative-based explanations were preferred on average on all questions.}
\label{tab:user-study-summary}
\resizebox{\linewidth}{!}{\begin{tabular}{@{}lll@{}}
\toprule
                                             & \multicolumn{2}{l}{\textbf{Average Rating}} \\
\textbf{Question}                            & \textbf{Narrative}      & \textbf{Plot}     \\ \midrule
From the explanation, I understand how the algorithm works.                    & \textbf{4.44} & 4.07 \\
The explanation is useful                    & \textbf{4.54}           & 4.07              \\
The explanation helps me know when I should trust the algorithm. & \textbf{3.86} & 3.09 \\
The explanation is clear and understandable. & \textbf{4.55}           & 3.57              \\
The explanation is sufficiently detailed.    & \textbf{4.17}           & 2.99              \\ \bottomrule
\end{tabular}}
\end{table}

==> CHI2024_workshop/intro.tex <==
\label{sec:intro}

%Explainability refers to the ability to explain or present model behavior (e.g. predictions) in human-understandable terms. 
In recent years, the demand for Explainable Artificial Intelligence (XAI) has increased, driven by concerns about the opacity and lack of interpretability of complex machine learning models~\cite{arrieta2020explainable, bhatt_explainable_2020}. 
%XAI is often offered as the answer to the black box problem and is broadly defined as “machine learning techniques that make it possible for human users to understand, appropriately trust, and effectively manage AI”~\cite{hbs2019}. 
%Despite years of research and application, the field of XAI still struggles to meet its goal of explainability, with resulting explanations requiring expert translation ~\cite{yang2023survey} or being better suited for use by ML experts \cite{bhatt_explainable_2020}. 
%For example, a common approach in XAI is SHapley Additive exPlanations (SHAP), which learns the marginal contribution that each feature makes to a given prediction. Despite the seemingly straight-forward nature of such feature contribution explanations, 
However, domain experts without ML experience still struggle to understand and use many ML explanations, which are often presented in a way that is not natural and human-readable \cite{bhatt_explainable_2020, jiang_two_2021, nyre-yu_considerations_2021, yang2023survey, zytek_sibyl_2021}. %miss examples 
%One possible solution to this challenge is to present explanations in a more natural, human-readable way. Prior attempts to reduce friction in explanation interpretation by non-experts have relied on either comprehensive onboarding efforts \cite{nyre-yu_considerations_2021}.
%, or manual, one-off interactions between data scientists and domain experts---each with their own drawbacks (citations).

Having proven useful in a variety of domains~\cite{chang2023survey}, Large Language Models (LLMs) offer a promising way to advance the field of XAI. In this paper, we investigate whether LLMs can improve explanations by transforming them into natural, human-readable narratives. In particular, LLMs' access to extensive background information may allow them to further ``explain explanations'' by offering context information.

LLMs may aid in XAI in many ways \cite{wuUsableXAI102024}. For example, some work has investigated using LLMs to directly explain ML models \cite{bhattacharjeeLLMguidedCausalExplainability2024, kroeger2023large} or to understand user questions to generate the appropriate explanation \cite{nguyen2023black, shenConvXAIDeliveringHeterogeneous2023, slack2023explaining}. In this work, we instead focus on using LLMs to transform existing ML explanations, generated by theoretically-grounded explanation algorithms such as SHAP \cite{lundberg2017unified}, into natural language narratives. 
%Existing work \cite{burton2023natural, nguyen2023black, slack2023explaining} has taken the first steps in this direction
We begin by proposing research directions we believe will further this goal, and then discuss our current progress on a few of these directions.


%we take the first steps into investigating the use of LLMs for XAI. Rather than using LLMs to directly explain ML models as previous work has done \cite{}, we seek to use LLMs only to transform existing ML explanations, generated by theoretically-grounded explanation algorithms, into naturally-worded narratives. We believe that this approach reduces the likelihood of introducing hallucinations, for more accurate explanations.

%The claim: 
%LLMs can be used for XAI to improve explanations by transforming them into natural narratives that users may prefer. However, further work and empirical evaluation is required to ensure they can do so consistently and accurately. 

%This work explores the use of LLMs to develop natural, human-readable narratives that frame model explanations pre-generated by theoretically-grounded XAI algorithms. %We focus on SHAP explanations which have been transformed to an interpretable forms by Pyreal, a system for generating a variety of interpretable ML explanations~\cite{zytek2023pyreal}.  %should we use pyreal or not?


% We build our narratives on top of Pyreal explanations, but introduce an additional, theoretically-grounded transformation to reduce the possibility of hallucinations---a common concern when applying LLMs. 

% 1. Why use pyreal instead of direct SHAP? (reason seems to be tied to reducing hallucinations because there's a transformation)--> this assumption is not grounded.

% 2. What to write: 
%     1) a parapgraph explaining why hallucinations are a concern
%     2) why pyrea is helpful in this, otherwise you cannot talk about hallucinations. 

% which are made interpretable through a theoretically-grounded transformation to reduce the opportunity for LLMs to introduce hallucinations. 

% Specifically, we investigate the effectiveness of LLMs in explaining through narratives the explanations 


% , rethinking explainability under a more ambitious scope. %LLMs possess the ability to communicate directly in expressive natural language.%, potentially addressing the longstanding challenges faced by the XAI field.

% Having LLMs generate explanation directly poses a risk of introducing hallucinations. For greater accuracy,

% have rapidly emerged as powerful tools in both academia and industry, demonstrating impressive capabilities to solve various tasks, contrasting with prior models confined to solving specific tasks 

% by representing explanations in a more natural, human-readable way through narratives. 
%With the advent of pre-trained language models, such as GPT (Generative Pre-trained Transformer)~\cite{radford2018improving} and BERT (Bidirectional Encoder Representations from Transformers)~\cite{devlin2018bert}, they are gaining popularity in both academia and industry. 



%Our novel contributions are as follows:
%\begin{itemize}
%    \item \textbf{Introduction of LLMs for natural, human-readable explanations.} This work introduces an initial investigation into employing LLMs to represent explanations as natural, human-readable narratives, improving on the readability of existing XAI approaches.
%    \item \textbf{Comparison of LLMs: }The paper conducts a comparative analysis of different LLM techniques, assessing their effectiveness in conveying natural, human-readable narratives.
%    \item \textbf{User Study:} A user study is conducted to address the question, 'Do users understand explanations obtained through LLMs better than traditional plot-based explanations?' Adding empirical insights, this study contributes to discussions on the practical effectiveness of LLMs in enhancing explainability. 
%\end{itemize}

%Through this work, we take the first steps into investigating and evaluating narrative explanations generated by LLMs from traditional SHAP explanations.



%The remainder of this paper is organized as follows: in Section~\ref{sec:background}, we delve into the background and introduce Pyreal. Section~\ref{sec:methods} outlines the methodologies employed to transform Sybil's explanations into natural, human-readable language. Moving on to Section~\ref{sec:results}, we showcase the outcomes derived from applying these methods across two distinct datasets, along with insights from the user study. Finally, Section~\ref{sec:conclusions} encapsulates the concluding remarks of this work, outlining our findings and charting the course for future directions in our research endeavors.

==> IEEE_Big_Data/body_first_submission.tex <==
\newcommand{\note}[1]{\textcolor{red}{#1}}
\newcommand{\narrator}{narrator}
\newcommand{\Narrator}{\textsc{Narrator}}
\newcommand{\grader}{grader}
\newcommand{\Grader}{\textsc{Grader}}

\newcommand{\Explingo}{\textsc{Explingo}}

\newcommand{\goldstandard}{exemplar}
\newcommand{\GOLDSTANDARD}{EXEMPLAR}
\newcommand{\GoldStandard}{Exemplar}


%\setlength{\belowcaptionskip}{-10pt}

\newcommand{\prompt}[1]{
    \begin{tcolorbox}[colback=gray!8, colframe=gray!80!black, width=\columnwidth, boxsep=1pt, left=-4pt, right=0pt, top=4pt, bottom=4pt]
    \noindent
    \begin{quote}
    #1
    \end{quote}
    \end{tcolorbox}
}



\section{Introduction}
% High level goal: produce and evaluate natural-language versions of traditional ML explanations. In this paper, rather than diving deep into the HCI question of how exactly these explanations are best disseminated, we instead focus on demonstrating that, given some small \goldstandard{} dataset of natural-language explanations created for some application, we are able to tune an LLM to create more explanations based on this \goldstandard{}.

Explanations of ML model predictions, such as those created by Explainable AI (XAI) algorithms like SHAP \cite{lundberg2017unified}, are important for making ML outputs usable for decision-making. It is difficult for users to make informed decisions using ML outputs without some explanation or justification of how ML model arrived at those. Past work \cite{lakkaraju_rethinking_2022, zytek_llms_2024} has suggested that some users may prefer explanations in a natural language format --- what we refer to in this paper as \textit{narratives}. Fig. \ref{fig:narrator-prompt-simple} shows an example of such a narrative. Such narratives offer many benefits: they align with how humans naturally communicate, allow users to glean key takeaways quickly, and are a first step in enabling interactive conversations where users can better understand models by asking follow-up questions.

Large Language Models (LLMs) 
%have a sufficient understanding and command of natural language to 
offer a promising way of generating such narratives.
%in a consistent and automated way. 
Past work has suggested different ways to do so. Some work \cite{bhattacharjeeLLMguidedCausalExplainability2024, kroegerAreLargeLanguage2023} uses LLMs directly to explain ML predictions, without use of traditional XAI algorithms. While these approaches offer promising paths towards novel explanations, they also risk introducing inaccuracy or hallucination in explanations. An alternative approach, and the one we focus on in this paper, is to use LLMs to transform existing ML explanations generated using traditional, theoretically grounded XAI approaches into readable narratives. 
%We pass an ML explanation in a text-based format, along with instructions on how to read it, and the LLM returns the information in the explanation in natural-language format. %As such, we take an explanation-transform approach \cite{zytek2023pyreal}.
%This builds on work in explanation transformation \cite{zytek2023pyreal} to improve the interpretablity of explanations.

% \begin{figure}[t!]
%     \centering
%     \begin{subfigure}[c]{\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{IEEE Big Data/ames_plot_sample.pdf}
%     \end{subfigure}

%     \vspace{.5em}
    
%     \raisebox{0.5\height}{\Large$\downarrow$}

%     \vspace{.5em}
    
%     % Subfigure 2: Nicely formatted text
%     \begin{subfigure}[c]{.9\linewidth}
%         \centering
%         \begin{minipage}{\linewidth}
%         \centering
%         \small
%             \textbf{``This house may sell for less because it is comparatively small, at around 850 square feet, and more than 90 years old. Despite the age, however, the house is in excellent shape, with condition rated at 8/10, which increases the predicted price by around \$13,000''}
%         \end{minipage}
%     \end{subfigure}
%     \caption{Example of transforming a traditional SHAP feature contribution explanation presented as a bar plot (top) into a human-worded, natural-language narrative (bottom). The SHAP value plot illustrates the impact of different features on the model's prediction for property valuation. %The negative contribution from the living area and the original construction date reflects a decrease in value. Conversely, the overall condition score of 8 contributes positively, adding around \$13k to the property's value.
%     The x-axis represents the dollar impact of each feature on the prediction, highlighting how different aspects of the property contribute to the estimated value.}
%     \label{fig:narrative-example}
% \end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/narrator_prompt_v2.pdf}
    \caption{Sample \Narrator{} inputs and outputs. The items in blue make up the prompt passed to the \Narrator{} to transform ML explanations into narratives for a house-pricing example. The item in green is a narrative version the \Narrator{} LLM may generate based on this prompt. Some components, like the output instructions, are provided by DSPy \cite{khattab2023dspycompilingdeclarativelanguage}.
    %This initial version of the prompt includes no hand-written narrative examples; in a subsequent version, we added hand-written examples of explanations and their corresponding narrative versions.
    %s along with the explanations that they explain. This improved the quality of narratives generted.
    }
    \label{fig:narrator-prompt-simple}
\end{figure*}

% \begin{figure}
%     \centering
%     \hspace*{-.5cm}
%     \includegraphics[width=1.05\linewidth]{IEEE Big Data/Main Process.pdf}
%     \caption{Summary of the inputs and outputs to the \Narrator{} and \Grader{} systems. The \Narrator{} takes in the parsed ML explanation, explanation format, and model context description and returns and narratives, which gets passed to the user. The \Grader{} generates grades based on this narrative, cross-referencing the information in the inputs as needed.}
%     \label{fig:process}
% \end{figure}

We seek to address two primary research questions:

\begin{enumerate}[left=0cm]
    \item Can LLMs effectively transform traditional ML explanations into high-quality narrative versions of explanations? these
\end{enumerate}

We address these questions with our two-part \Explingo{} system. To address the first question, we develop an LLM-based \Narrator{} that transforms SHAP explanations from diverse datasets into narratives. We then investigate what metrics may be of value to assess the quality of narratives, and auto-grade the generated narratives using our \Grader{} to address the second question. Automatically grading narratives is helpful not only for tuning and evaluating the system, but also can be used as guardrails in deployment by hiding any narratives that are not of sufficient quality.

We note that users across different domains may have significantly different preferences for how these narratives should look. Some factors --- like the fact that narratives should accurately represent the original explanation and not be unnecessarily long --- are fairly universal. On the other hand, other factors are highly subjective. Some users may wish for a narrative that includes very precise and technical details, while others prefer more general information. 
%Some applications may require formal, technical descriptions while others benefit from more casual tones. 
In this paper, we aim to generate narratives that match the style of some small, user-provided \goldstandard{} dataset of narratives. Our objective is to create a system where, for any new application, a user can write a small number of sample narratives (around three to five) and get high-quality narrative versions of future ML predictions that mimic the style of those samples.
%and evaluating narratives based on this \goldstandard{}.

Our key contributions from this work are:
\begin{itemize}
    \item We present our \Narrator{} system that transforms ML explanations into user-readable narratives.
    \item We develop an independent, automated \Grader{} system that assesses the quality of the generated narratives.
    \item We curated a sample set of nine \goldstandard{} dataset that contain narratives for four public datasets, that can be used for future narrative generation tuning and evaluation work. These datasets are public and can be accessed here: \url{https://github.com/sibyl-dev/Explingo}.
    \item We provide a comprehensive set of experiments to demonstrate the impact of different prompting and few-shot strategies on narrative generation, and evaluate potential sources of reduced narrative quality.
    \item Our system has been integrated in an open-source library here: \url{https://github.com/sibyl-dev/pyreal}.
\end{itemize}

\section{Background}
SHAP values \cite{lundberg2017unified} are a popular way to explain ML model predictions in terms of feature contributions. In these explanations, every feature is given a positive or negative value representing how much it increased or decreased the model's prediction on a specific input. Past work  has suggested these explanations are popular among users, but may be difficult for some user groups to parse \cite{zytek_sibyl_2021, suh_more_2024, bhatt_explainable_2020, jiang_two_2021, yang2023survey}. 

Past work has aimed to apply LLM's language-processing capabilities to XAI problems in different ways. Some work \cite{nguyen2023black, shenConvXAIDeliveringHeterogeneous2023, slack2023explaining} has focused on using LLMs at the input stage, taking in user questions and generating appropriate explanations to answer them. Other work \cite{bhattacharjeeLLMguidedCausalExplainability2024, kroegerAreLargeLanguage2023} has sought to use LLMs directly to generate explanations of model logic. 

In this paper, we instead build on work seeking to transform existing ML explanations into readable narratives. Burton et al. \cite{burton2023natural} used an LLM fine-tuned on a dataset of natural-language explanations to produce fluent and accurate narratives. Guo et al. \cite{guoAdaptingPromptFewshot2023} proposes a few-shot table-to-text generation approach that uses unlabeled domain-specific knowledge to convert tables into natural-language descriptions. We extend these works through an alternative scoring method based on a specific set of metrics, and use an approach based purely on a mix of manual and optimized prompting. 

Past work \cite{guo_evaluating_2023, bai_benchmarking_2023, chen_exploring_2023, ji_exploring_2023} has also looked into using LLMs to evaluate LLM outputs, in order to reduce effort and time required from a potentially small group of human users. Fu et al. \cite{fu_gptscore_2023} found that GPT-3 was able to effectively evaluate the quality of LLM-generated text based on a wide variety of metrics such as correctness, understandability, and diversity. Wang et al. \cite{wang_is_2023} similarly found that chat GPT is able to achieve state-of-the-art correlation with human graders. Liu et al. \cite{liu_g-eval_2023} found that advanced prompting techniques such as chain-of-thought prompting can further improve correlation between LLM and human grades. We applied these insights to optimize and evaluate our LLM-generated narratives using an LLM-based metric grader, eliminating the need for human graders and enabling evaluation across a wider range of domains without relying on domain experts.
%We leveraged these findings in order to tune and evaluate our LLM-generated narrative explanations based on grades from an LLM-based metric grader, thus removing the need for time from human graders, and allowing us to evaluate on a larger range of domains, without the need for domain experts. \note{rewrite paragraph} 


\section{The \Explingo{} System: \Narrator{} and \Grader{}}
To transform XAI explanations into narratives, the \Explingo{} system includes two sub-systems:
1) \Narrator{}: a system to transform traditional explanations of ML model predictions into accurate, natural narratives.
2) \Grader{}: a metric grading system to assess the quality of narratives. 
% The inputs and workflow of these systems are summarized in Fig. \ref{fig:process}.

\subsection{\Narrator{}: Transforming ML Explanations to Narratives}

Transforming traditional ML model explanations into readable narratives offers several potential benefits. First, these narratives allow key takeaways to be read quickly. Second, they are often the most natural format for parsing information for many users, who may prefer them to graphs or have difficulty understanding graphs that are not visualized effectively. Finally, offering narrative versions of explanations is the first step to allowing for full ``conversations'' with ML models, with users able to ask follow-up questions in natural-language and receive answers in kind.

The \Narrator{} is an LLM model, in our case GPT-4o, that is prompted to generate a narrative. The basic prompt is composed of four components: a base prompt, a definitions of the input component structure, three specific explanation components (the ML explanation, the explanation format, and the context description), and output instructions. The prompt is then concluded with \textbf{Narrative:} invoking the LLM to start narrating. The first four blocks in Figure~\ref{fig:narrator-prompt-simple} show an example prompt that follows this structure. As described in depth later, we additionally pass selected example narratives that help the \Narrator{} customize its narratives for specific applications. 

%``\textit{The model looked at the living area of the house, which is 854 square feet. Based on this information, it contributed a decrease of \$21,929 to the predicted house price. In simpler terms, the smaller living area of the house is leading to a lower estimated price compared to other factors the model considered.}''

% to the \Narrator{} LLM, formatted in a prompt to generate a narrative. Fig. \ref{fig:process} shows an example of inputs to the \Narrator{}.

The \textbf{explanation} --- for example, a SHAP feature contribution explanation, as we focus on in this paper --- is generated using some external library. We then parse this explanation into a consistent format, depending on the explanation type. For the SHAP explanation, we select the $N$ most contributing features by absolute value, and parse them in sorted order into the following format: 

\noindent\textit{(feature name 1, feature value 1, SHAP contribution 1), (feature name 2, feature value 2, SHAP contribution 2), \dots }

%\noindent For example, the data in Fig. \ref{fig:narrative-example}, where $N=3$, would be parsed as: \textit{(Living area square feet, 854, -21929),(Original construction date, 1929, -13746), (Overall condition, 8, 14928)}

% The number of features $N$ is user-selected, and will depend on the requirements of the application. 

In addition to the explanation, the \narrator{} takes in a brief \textbf{explanation format} describing how to parse the given explanation. Passing this format description separately makes the system generalizable  to any kind of ML explanation that can be expressed in text. Moreover, it allows the explanation to be customized for additional information to be passed.
%We use:

%\noindent\textit{SHAP feature contribution in (feature\_name, feature\_value, contribution) format}


% ; for example, for SHAP feature contributions, we could also pass the average feature value to add more information.

Finally, we write a brief description of the \textbf{context} of the explanation --- generally, what the ML model being explained is predicting. For SHAP explanations, this helps provide units to the contributions. 

The last box in Fig.~\ref{fig:narrator-prompt-simple} shows an example of the \Narrator{}'s output narrative.
%Fig.~\ref{fig:narrator-prompt-simple} shows a simple example of the \Narrator{} input. When supplying the \narrator{} with the given prompt, it generates the following example:
%``\textit{The model predicts the house price based on several key features. The above ground living area, which is 2090 square feet, contributes significantly to increasing the price by 16382.07 units. The second floor area, measuring 983 square feet, also adds a substantial 16216.99 units to the price.}''



%Fig. \ref{fig:narrator-prompt-simple} shows examples of all these inputs.
%For the example in Fig. \ref{fig:narrative-example}, this may look like ``\textit{the model predicts house prices}''.

% So how do we know if these narrative are good?
Once the \Narrator{} generates narratives, we want to assess if these narratives are high-quality and expressing the right information. This is where the \Grader{} plays a role.

% \begin{table}[ht]
% \centering
% \caption{SHAP Feature Contributions for House Price Prediction}
% \begin{tabular}{p{.25\linewidth}p{.6\linewidth}}
% \toprule 
% \textbf{Explanation} & (Above ground living area square feet, 854, -21929), (Original construction date, 1929, -13746), (Overall condition of the house, 8, 14928) \\
% \textbf{Explanation Format} & SHAP feature contribution in (feature\_name, feature\_value, contribution) format \\
% \textbf{Context} & The model predicts house prices \\
% \bottomrule
% \end{tabular}
% \label{tab:shap_contributions}
% \end{table}

\begin{table*}[t]
\centering
\caption{Summary of \goldstandard{} datasets. In the Ames Housing Dataset \cite{de_cock_ames_2011}, each row represents one house, with 79 input features. The label to be predicted is the price the hold sold for. The Student Performance Dataset \cite{cortez_using_2008} includes 30 features, and each row represents a student. The label to be predicted is whether the child will pass or fail a class. The Mushroom Toxicity Dataset \cite{misc_mushroom_73} has 22 features about different specifies of mushrooms, and the predicted label is whether the mushroom is poisonous or not. Finally, the PDF Malware Dataset \cite{issakhani_pdf_2022} has 37 features about different PDFs, and the prediction label is whether the PDF contains malware. }
\label{tab:datasets}
\begin{tabular}{p{.07\linewidth}p{.14\linewidth}cp{.63\linewidth}}
\toprule 
ID & Dataset & \# of Entries & Sample Narrative \\
\midrule 
House 1    &  Ames Housing  & 35 &    The relatively smaller above ground living space in this house reduces its predicted price by about \$12,000. The lower-than-average material rating also reduced the house price by about \$10,000.         \\
House 2     &  Ames Housing & 22 &  The SHAP value indicates that the house price decreases because the above ground living area is 1256 sq ft and the material quality is rated 5.              \\
House 3     &   Ames Housing  & 22 &  This house is cheaper because it has less above ground living space (size=1256) and has lower material quality (rating=5).                \\
Mush 1     & Mushroom Toxicity & 30 &     This mushroom is more likely to be poisonous because its foul odor, silky stalk surface, and chocolate spore print color. Be careful!             \\
Mush 2     & Mushroom Toxicity & 30 &    The absence of odor and broad gill size suggest the mushroom is less likely to be poisonous, but the brown spore print indicates a higher risk of toxicity.          \\
PDF 1      & PDF Malware & 30 &    The PDF file is more likely to contain malware because it has a larger metadata size (262 KB), a larger total size (74 KB), and no Javascript keywords.             \\
PDF 2      & PDF Malware & 30 &  The large metadata size (180 KB), the large total size (7 KB), and fewer objects suggest the PDF contains malware.  \\
Student 1 & Student Performance & 30 & We believe this child is less likely to pass because they do not have family support, and we have seen that male students tend to be more likely to fail. \\
Student 2 & Student Performance & 30 & The lack of family support, and the sex (male) suggest the student is less likely to pass the class. But, the lack of a romantic relationship indicates an higher probability of passing. \\ \bottomrule
\end{tabular}
\end{table*}


%\begin{figure}
%\centering
   % \prompt{
 %   How accurate is the information in the narrative, based on the explanation given? A narrative can achieve a grade of 4 even if it is missing information as long as everything in the narrative is correct. Make sure the contribution direction is correct - positive contributions increase the output, negative contributions decrease the output.
%    \newline
    
   % \textbf{Explanation Format:} SHAP feature contribution in (feature\_name, feature\_value, contribution) format
    
   % \textbf{Explanation:} (Living area square feet, 854, -21929)
    
   % \textbf{Narrative:} The model looked at the living area of the house, which is 854 square feet. Based on this information, it contributed a decrease of \$21,929 to the predicted house price. In simpler terms, the smaller living area of the house is leading to a lower estimated price compared to other factors the model considered.
     
   % \textbf{Rubric:} 0 - Contains one or more errors in value or contribution direction. 1 - Contains no errors, but may be missing information.
    
   % \textbf{Assessment: }
   % }
%\caption{Prompt passed to the \Grader{} to evaluate the accuracy of the narrative based on Fig~\ref{fig:narrative-example} and Fig~\ref{fig:narrator-prompt-simple} examples.}
%\label{fig:grader-prompt-simple}
%\end{figure}

    % \prompt{
    % \textbf{Question:} How accurate is the information in the narrative, based on the explanation given? A narrative can achieve a grade of 4 even if it is missing information as long as everything in the narrative is correct. Make sure the contribution direction is correct - positive contributions increase the output, negative contributions decrease the output.
    % \newline
    
    % \textbf{Explanation format:} (feature\_name, feature\_value, SHAP contribution). 
    
    % \textbf{Explanation:} [[EXPLANATION]]
    % \newline
    
    % \textbf{Narrative:} [[NARRATIVE]]
    % \newline
    
    % \textbf{Rubric:} 0 - Contains one or more errors in value or contribution direction. 1 - Contains no errors, but may be missing information.
    % \newline
    
    % \textbf{Assessment: }
    % }

\subsection{\Grader{}: Assessing the Quality of Narratives}
To assess the quality of narratives, we adapted metrics proposed in \cite{zhouEvaluatingQualityMachine2021}, which include:
\begin{itemize}
    \item \textit{Accuracy}: how accurate the narrative is to the original ML explanation.
    \item \textit{Completeness}: how much of the information from the original ML explanation is present in the narrative.
    \item \textit{Fluency}: how naturally-worded the narrative is.
    \item \textit{Conciseness}: how long the narrative is considering the number of features in the explanation.
\end{itemize}

% Other metrics such as METEOR \cite{banerjee-lavie-2005-meteor} have been used to evaluate LLM output quality in previous work. However, to compute these metrics, we need a ground-truth label for every narrative. In real-world deployment, we have not have these labels available, making these metrics impractical for use as guardrails. With our automated \Grader{} system, metrics can be computed without ground-truth labels, making them valuable in deployment.

While there are other metrics that can be included, for the presentation of the \Grader, we focus on these four. The challenge with these metrics is that they are time consuming to manually compute, and manual assessment could introduce human bias into the evaluation.

Our \Grader{} automatically evaluates the quality of the narrative by prompting an independent LLM, GPT-4o in our case, to consider the ML explanation and the generated narrative and assign a value to the respective metric. Fig. \ref{fig:accuracy-prompt} shows an example of a \Grader{} prompt evaluating the accuracy metric. In summary, it takes in the input and output of the \Narrator{} along with a rubric criteria, and comes up with a score depending on which metric it is asked to assess. In Fig. ~\ref{fig:accuracy-prompt}, the \grader{} return will return either \textbf{1}, indicating an accurate narrative, or \textbf{0} for an inaccurate narrative.
Straight out-of-the-box, it can be difficult for LLMs to produce the exact desired output. %, as LLMs tend to add superfluous words. 
Section \ref{sec:metrics} goes into details about how we tuned, validated, and used the \Grader{} system.

It is worth noting that in previous work, metrics such as METEOR~\cite{banerjee-lavie-2005-meteor} have been used to evaluate LLM output quality. However, to compute these metrics, we need a ground-truth label for every narrative. In real-world settings, we do not have these labels available, making it impractical in deployment. With \Grader, we alleviate this barrier.

Putting effort into developing and validating a \Grader{} system offers several benefits. A well-validated grader can quickly adapt to a large variety of domains and dramatically reduce human-effort required to evaluate narratives. It can also be used as part of the finetuning process, as certain LLM optimization functions like bootstrapping few-shot examples optimize based on automated evaluation functions. Finally, and perhaps most importantly, a well-validated grader can be used as a guardrail in live deployment scenarios --- rather than risking showing inaccurate or low-quality narratives to users, a system can automatically revert to the default, graph-based ML explanation in situations where the generated narrative scores are unacceptable.

Narratives can be written in numerous ways and the desired style of narratives is highly subjective. Therefore, we introduce the concept of an \goldstandard{} dataset, which is a small dataset provided by the user containing high-quality examples of narratives. We then tune the \Grader{} according to the \goldstandard{}s. With the \Grader{} and \goldstandard{}s, we can steer the \Narrator{} to transform the explanation into narratives that match the style of the \goldstandard{}s.

%We chose to develop our own custom \Grader{} rather than relying on existing metrics such as METEOR \cite{banerjee-lavie-2005-meteor} scores as these existing metrics rely on comparisons to a ground-truth for every input; in order to be use as a guardrail for live deployment, we need metrics that can grade without access to such information.

% Our \Grader{} takes in a narrative explanation, along with the key inputs described above (the explanation, explanation format, and context), as well as some tuning parameters such as sample \goldstandard{} narratives, and returns grades on each of a set of metrics. Most of these metrics are graded by an LLM internally. 

% \begin{figure*}[tb!]
%     \centering
%     \begin{lstlisting}[language=Python]
%     "explanation": "(odor, foul, 0.24), (stalk-surface-above-ring, silky, 0.10)",
%     "explanation_format": "(feature_name, feature_value, SHAP contribution)",
%     "context": "The model predicts whether a mushroom is poisonous",
%     "narrative": "This mushroom is more likely to be poisonous because its foul odor and silky stalk 
%                   surface. Be careful!" \end{lstlisting}
%     \caption{Sample entry from the \textbf{mush 1} evaluation dataset. \note{Once process figure is added, we may be able to remove this figure}}
%     \label{fig:eval-example}
% \end{figure*}

\begin{table}[t]
\centering
\caption{Summary of metric validation datasets for the accuracy and completeness metrics. For accuracy, we include both complete and incomplete narratives to ensure they are both be rated as accurate.}
\label{tab:validation-datasets}
\begin{tabular}{@{}lp{4cm}cc@{}}
\toprule
Metric       & Type                                                    & Rubric Grade & Count \\ \midrule
Accuracy     & Accurate with all values                                       & 1            & 15                                 \\
             & Accurate with some values                                     & 1            & 8                                 \\
             & Accurate with approximate values                            & 1            & 8                                  \\
             & Error in values                                             & 0            & 6                                 \\
             & Error in contribution direction                             & 0            & 7                                 \\
            & Total & & 44 \\ \midrule
Completeness & \raggedright All features, values, and contributions                     & 2            & 3                                 \\
             & \raggedright All features, values, and contribution directions           & 2            & 4                                 \\
             & \raggedright All features, but not all values or contribution directions & 1            & 9                                \\
             & Missing one or more features                                & 0            & 10                                 \\ 
             & Total & & 26 \\ \bottomrule
\end{tabular}
\end{table}


\section{\GoldStandard{} and Evaluation Datasets} \label{sec:datasets}
%For this work, we created and used a starting set of nine datasets for use as \goldstandard{}s and for \Narrator{} evaluation, summarized in Table \ref{tab:datasets}. These datasets used data from four publicly available ML datasets. 
For this work, we picked four publicly available ML datasets. We selected these datasets to include a wide variety of contexts ranging from predicting prices of houses to predicting toxicity of mushrooms. From these we created \goldstandard{}s for generating narratives. To create an exemplar dataset, we pick a data point and form an entry.  Each entry represents one model prediction on one data point. Each entry includes a SHAP explanation, an explanation format descriptor, and a brief context sentence describing what the model task is (e.g. predicting house prices). In total we created nine exemplar datasets for use as summarized in Table \ref{tab:datasets}. 
%Each of the nine datasets we created includes between 22 and 35 entries. 

\textbf{Hand-written narratives:} For each \goldstandard{} dataset, we picked a few entries and created hand-written narratives given their SHAP explanations. These narratives were written by different authors and had a distinctive wiriting style. Different contexts (i.e., what model predicts) require some amount of customization to achieve the best possible narratives automatically from an LLM. These hand-written narratives thus become a foundational piece in our system. To use our system for a new context (a new model), the user would create a few entries and write narratives with their preferred style and information. These entries can then be used to optimize our system to provide better narratives specific for the context and users' preferred narration style. 

%As discussed above, narrative quality is a highly subjective and context-dependent concept; therefore, rather than attempting to generate all-purpose gold-standard narratives, we instead aim to generate explanations that mimic the style of small, application-specific \goldstandard{} datasets. 
%Rather than require users to manually evaluate and adjust prompts for each new application, they can simply write out a small number of narratives based on a few possible explanations, and the \Narrator{} and \Grader{} will both use these examples for narrative generation and grading, respectively. 
%Fig. \ref{fig:eval-example} shows an example of one entry from one of these datasets.

%From each dataset, we randomly removed 5 of the human-labeled entries (ie. those with narratives) to use as human-labeled few-shot examples, as well as another 5 random entries to use as inputs for the bootstrapping additional few-shot examples. We then generated narrative explanations based on the remaining entries, and scored them using our metric scoring functions.

%Three of our \goldstandard{} datasets used data from the Ames Housing Dataset \cite{de_cock_ames_2011}; two each came from the Student Performance Dataset \cite{cortez_using_2008}, Mushroom Toxicity \cite{misc_mushroom_73} dataset, and PDF Malware dataset \cite{issakhani_pdf_2022}.

%\section{Experiment Setup} \label{sec:exp-setup}
%In this work, we used DSPy\footnote{https://github.com/stanfordnlp/dspy}, an open-source LLM programming framework. DSPy enabled us to experiment with different LLM steering and tuning approaches and run evaluations in a structured manner. The prompts we show in Sections \ref{sec:metrics} and \ref{sec:methods} are the output from DSPy's programming\footnote{The DSPy signatures and inputs used can be seen in our experiment code at https://github.com/sibyl-dev/Explingo}.

%We experimented with multiple API-based LLM models for the explanation transformation process including GPT-3.5, GPT-4o, Claude, Gemma, and Mistral, as we determined these large models could complete the task effectively with minimal tuning. Based on initial results, we decided to run experiments using GPT-4o. \note{If we do use a local LLM, talk about that here}
%To investigate whether our findings can extend to smaller models, we additionally ran experiments with a local LLM \note{elbaorate}
%with two LLMs, one API-based and one local. For the API-based LLM, we used GPT-4O. For the local API, we used X.


%In the next section, we introduce our metrics, and discuss our metric scoring functions.


\section{Automated Grading of Narratives} \label{sec:metrics}
%Zhou et al. \cite{zhouEvaluatingQualityMachine2021} suggested a diverse set of metrics to evaluate the quality of XAI. We adapted this list for specific use on narrative explanations. 
In this paper, we focus on steering an LLM to transform explanations into narratives that are optimized on four metrics: accuracy, completeness, fluency, and conciseness. 
%Previously \cite{zytek_llms_2024}, we manually rated narratives on these metrics. However, this is a time consuming process that is not practical for large-scale evaluations and optimizations. Therefore, we sought to develop automated methods for effectively scoring narratives on these four metrics. 
Scoring conciseness is a straightforward computation based on word-count; the other metrics were graded using a GPT-4o LLM \Grader{}. We had the LLM grade each narrative 5 times and then took the average grade. To ensure consistency in grades, we would check and alert if any two of these 5 grades varied by more than 1; however, this alert was never raised during our experimentation. 

%All metrics are scaled to be graded between 0 and 4 to keep equal weighting being metrics (which can then be adjusted with weighting parameters). 
Our total grade $G$ for a narrative is then computed by weighting and aggregating all metrics with the following equation:
\begin{equation}
    G = \alpha_a A + \alpha_f F + \alpha_c C + \alpha_s S
\end{equation}
where $A$ is the Accuracy grade, $F$ is the Fluency grade, $C$ is the Completeness grade, $S$ is the conciseness grade, and the $\alpha$ parameters are weighting constants. 


As described in more depth below, accuracy is scored on 2-point 0/1 scale, the completeness is scored on a 3 point 0/1/2 scale, and fluency and conciseness are scored between 0 and 4. For our experiments, we therefore equally weighted all metrics by setting $\alpha_a=4, \alpha_c=2, \alpha_f=\alpha_s=1$, and report these weighted metric values in our results.

In running and optimizing LLMs, we used DSPy\footnote{https://github.com/stanfordnlp/dspy} \cite{khattab2023dspycompilingdeclarativelanguage}, an open-source LLM programming framework. 
%DSPy enabled us to experiment with different LLM steering and tuning approaches and run evaluations in a structured manner. 
The prompts we show in this and later sections are the output our DSPy program\footnote{The DSPy signatures and inputs used can be seen in our experiment code at https://github.com/sibyl-dev/Explingo}.

In addition to the information shown in the prompts presented through this section, the prompt given to the \Grader{} LLM also included instructions on how to parse the input components (as in the ``Definitions'' box of Fig. \ref{fig:narrator-prompt-simple}), and instructions to return only a single number from the rubric, which was then parsed out as the grade.

In the rest of this section, we introduce the metrics we used to evaluate narratives, and our process for developing and validating our \Grader{}.

\begin{figure}[t]
    \centering
    \prompt{
    \textbf{Question:} How accurate is the information in the narrative, based on the explanation given? A narrative can achieve a grade of 4 even if it is missing information as long as everything in the narrative is correct. Make sure the contribution direction is correct - positive contributions increase the output, negative contributions decrease the output.
    \newline
    
    \textbf{Explanation format:} (feature\_name, feature\_value, SHAP contribution). 
    
    \textbf{Explanation:} [[EXPLANATION]]
    \newline
    
    \textbf{Narrative:} [[NARRATIVE]]
    \newline
    
    \textbf{Rubric:} 0 - Contains one or more errors in value or contribution direction. 1 - Contains no errors, but may be missing information.
    \newline
    
    \textbf{Assessment: }
    }
    \caption{Prompt passed to the \Grader{} to compute the accuracy metric. The LLM is first told how to parse the input components (as in the ``Definitions'' box of Fig. \ref{fig:narrator-prompt-simple}), and instructed to return only a single number from the rubric. Experiments suggested that asking for a grade from a 2-point rubric resulted in better performance than a simple yes/no question. 
    %By explicitly telling the \Grader{} LLM to pay attention to contribution directions and grade highly even on missing data, we were able to improve \Grader{} performance in areas where it appeared to underperform.
    }
    \label{fig:accuracy-prompt}
\end{figure}

\subsection{Accuracy} 
The accuracy metric evaluates if the information in the narrative is correct based on the input explanation. For example, in an accurate narrative, all feature values, SHAP feature contribution values, and  contribution directions (positive or negative) are correct. 
% We note that, in keeping this metric separate from the completeness metric, incomplete narratives (ie. narratives that do not include all information from the original explanation) can still be considered accurate. 
Narratives that do not mention all features are still considered accurate. 
This metric was scored on a Boolean scale of 0 (inaccurate) or 1 (accurate).

Accuracy is scored by the \Grader{} by passing in a prompt to the LLM. This prompt includes the input ML explanation, the explanation format, and the narrative to grade, and asks the LLM whether or not the narrative was accurate.
%This prompt contained the explanation format, explanation, narrative and a rubric and a question at the beginning to ask for an assessment of correctness. This question, that we ask at the beginning, needs to be fine tuned to make our scoring function in the GRADER to give…

In order to tune and validate the prompt passed into our \Grader{} for accuracy, we developed a metric validation dataset of 44 explanation-narrative pairs, along with human-labeled accuracy grades. These examples contained randomly selected SHAP explanations, with narratives. These narratives were intentionally written to span five levels of accuracy, as summarized in Table \ref{tab:validation-datasets}. 

We started with a basic prompt (\textit{How accurate is the information based on the explanation given?}), passed the dataset entries to the \Grader{}, and evaluated its performance on narratives of each level of accuracy. We used these results to iteratively adjust the prompt. For example, we saw that the \Grader{} incorrectly considered narratives that were accurate but did not include all feature values from the input explanation as inaccurate, and added instructions to the prompt accordingly. Fig. \ref{fig:accuracy-prompt} shows our final version of the prompt.

%: complete and correct narratives (grade=1), incomplete and complete narratives (grade=1), narratives that use approximate values (grade=1, though we note that the grade for this category is context-dependent), narratives that contain errors in values, and inaccurate narratives that contain errors in contribution direction (ie, saying a feature ``increased the model's prediction'' when the feature's contribution was negative). The full spread of narratives across this metric validation dataset can be seen in Table \ref{tab:validation-datasets}.

%We additionally generated a smaller tuning dataset of 10 narratives (2 from each category) to tune the prompts given to the \Grader{} LLM. 
%After experimentation, we determined that the highest performance was achieved when asking the LLM to grade the accuracy on a 2-point rubric (compared to asking a yes/no question), 
%Fig. \ref{fig:accuracy-prompt} shows our final prompt.

\begin{figure}
    \centering

    \prompt{
\textbf{Question:} How completely does the narrative below describe the explanation given? 
\newline

\textbf{Explanation format:} (feature\_name, feature\_value, SHAP contribution). 

\textbf{Explanation:} [[EXPLANATION]]
\newline

\textbf{Narrative:} [[NARRATIVE]]
\newline

\textbf{Rubric:} 0 - One or more feature names from the explanation are not mentioned at all in the narrative. 1 - All features are mentioned, but not all feature values and/or contribution directions. 2 - All features are mentioned, and for each feature, includes at least an approximation of the feature's value and contribution direction.
\newline

Start by listing out all the features in the explanations, and then determine if every feature is present in the narrative, along with its value and contribution direction. 
\newline

\textbf{Assessment:}
}
    \caption{Prompt passed to the \Grader{} to compute the completeness metric. 
    %Based on experimenting with a smaller tuning dataset, we found that basic prompting was insufficient for a performant completeness scoring function. Through experimentation, we determined that a chain-of-thought \cite{wei_chain--thought_2023} approach worked best.
    }
    \label{fig:completeness-prompt}
\end{figure}


\newcommand{\shadecell}[1]{\cellcolor[gray]{\ifnum#1>5 0.65\else\ifnum#1>2 0.9\else 0.95\fi\fi} #1}

\begin{table}[b]
\centering
\caption{Agreement between \Grader{} and human-labeled validation set for Accuracy (left) and Completeness (right).} \label{tab:accuracy_and_completeness}
\begin{tabular}{cccc}
   & & \multicolumn{2}{c}{\textbf{\Grader{}}} \\ 
  & & 0 & 1 \\ \midrule
  \multirow{3}{*}{\rotatebox{90}{\textbf{Human}}} & 0 & \shadecell{12} & \shadecell{1} \\
  & 1 & \shadecell{2} & \shadecell{29} \\ \\ \bottomrule
\end{tabular}
\hspace{1cm}  % Adjust space between the two tables
\begin{tabular}{ccccc}
   & & \multicolumn{3}{c}{\textbf{\Grader{}}} \\ 
  & & 0 & 1 & 2 \\ \midrule
  \multirow{3}{*}{\rotatebox{90}{\textbf{Human}}} 
  & 0 & \shadecell{10} & \shadecell{0} & \shadecell{0} \\
  & 1 & \shadecell{0} & \shadecell{8} & \shadecell{1} \\
  & 2 & \shadecell{0} & \shadecell{1} & \shadecell{6} \\ \bottomrule
\end{tabular}

\end{table}

% \Grader{}




% \begin{figure}[h]
%     \centering
%     \noindent\fbox{%
%     \parbox{\columnwidth}{% Adjust the width to fit within the column
%     \vspace{-2pt} % Adds some vertical space inside the box
%     \begin{tabular}{p{2cm} p{6.2cm}} % Adjusted widths for two-column format
%     \textbf{Question:} & How accurate is the information in the narrative based on the explanation given? 
%     \\
%     & A narrative can achieve a grade of 4 even if it is missing information. Everything in the narrative must be correct. \\
%     & Ensure contribution direction is correct: Positive contributions increase the output, and negative contributions decrease the output. \\[12pt]
    
%     \textbf{Explanation Format:} & (feature\_name, feature\_value, SHAP contribution) \\[10pt]
    
%     \textbf{Explanation:} & [[EXPLANATION]] \\[10pt]
    
%     \textbf{Narrative:} & [[NARRATIVE]] \\[10pt]
    
%     \textbf{Rubric:} & 
%     \textbf{0} - Contains one or more errors in value or contribution direction. \textbf{4} - Contains no errors, but may be missing information. \\[10pt]
    
%     \textbf{Assessment:} & [[ASSESSMENT]] \\
%     \end{tabular}
%     \vspace{3pt} % Adds some vertical space inside the box
%     }}
%     \caption{Assessment of Narrative Accuracy Based on SHAP Explanation}
%     \label{fig:accuracy-metric}
% \end{figure}

\begin{table*}[]
\centering
\caption{Average fluency scores for each dataset based on each \goldstandard{} dataset. We expect the scores down the diagonal (highlighted) to be the highest. The actual highest scores are per row are bolded.}
\label{tab:fluency-validation}
\begin{tabular}{lccccccccc}
\hline
                   & \multicolumn{9}{c}{\textbf{\GoldStandard{}}}                                                                                                                                                                                                                                                                                                                             \\
                   & \textbf{House 1}                      & \textbf{House 2}                      & \textbf{House 3}                      & \textbf{Mush 1}                       & \multicolumn{1}{l}{\textbf{Mush 2}}   & \textbf{PDF 1}                        & \multicolumn{1}{l}{\textbf{PDF 2}}    & \textbf{Student 1}                    & \multicolumn{1}{l}{\textbf{Student 2}} \\ \hline
\textbf{House 1}   & \cellcolor[HTML]{EFEFEF}\textbf{4.00} & 3.45                                  & 3.75                                  & 0.90                                  & 1.00                                  & 1.00                                  & 0.25                                  & 0.30                                  & 1.65                                   \\
\textbf{House 2}   & 3.00                                  & \cellcolor[HTML]{EFEFEF}\textbf{4.00} & 3.67                                  & 1.83                                  & 1.33                                  & 1.00                                  & 0.08                                  & 0.08                                  & 1.67                                   \\
\textbf{House 3}   & 2.31                                  & 3.38                                  & \cellcolor[HTML]{EFEFEF}\textbf{4.00} & 1.46                                  & 0.15                                  & 1.62                                  & 0.15                                  & 0.31                                  & 0.46                                   \\
\textbf{Mush 1}    & 0.00                                  & 0.18                                  & 1.55                                  & \cellcolor[HTML]{EFEFEF}\textbf{4.00} & 3.27                                  & 0.64                                  & 0.00                                  & 0.91                                  & 1.27                                   \\
\textbf{Mush 2}    & 0.00                                  & 0.00                                  & 0.00                                  & 3.36                                  & \cellcolor[HTML]{EFEFEF}\textbf{4.00} & 0.45                                  & 0.55                                  & 0.64                                  & 2.36                                   \\
\textbf{PDF 1}     & 0.00                                  & 0.11                                  & 2.11                                  & 3.22                                  & 0.78                                  & \cellcolor[HTML]{EFEFEF}\textbf{4.00} & 3.78                                  & 0.44                                  & 0.44                                   \\
\textbf{PDF 2}     & 0.00                                  & 0.00                                  & 0.00                                  & 0.44                                  & 2.11                                  & 3.78                                  & \cellcolor[HTML]{EFEFEF}\textbf{3.89} & 0.00                                  & 1.89                                   \\
\textbf{Student 1} & 0.00                                  & 0.07                                  & 0.37                                  & 0.70                                  & 0.20                                  & 0.03                                  & 0.00                                  & \cellcolor[HTML]{EFEFEF}\textbf{3.97} & 3.87                                   \\
\textbf{Student 2} & 0.00                                  & 0.50                                  & 0.00                                  & 0.36                                  & 1.50                                  & 0.07                                  & 0.64                                  & 3.79                                  & \cellcolor[HTML]{EFEFEF}\textbf{4.00}  \\ \hline
\end{tabular}
\end{table*}

The final version of our \Grader{} achieved 93\% accuracy, in terms of agreement with the human-labeled grade on the validation dataset. A more detailed analysis of these results is shown in Table \ref{tab:accuracy_and_completeness}.


%This metric is scored on a 3-point rubric with the following values. 0: One or more errors. 2: No errors but worded in a misleading way (for example, referring to a quality of 5/10 as ``high quality'' or using the phrase ``suprisingly'' when referring to intuitive information). 4: All information provided is correct.

%We graded this metric using our \Grader{} LLM on the rubric above with the following prompt: \textit{Everything said in the narrative is accurate based on the explanation.}

\subsection{Completeness}
The completeness metric grades how much of the information from the input ML explanation is present in the narrative. For our experiments, we define a complete explanation as one that 1) mentions all features and their values from the ML explanation and 2) mentions the contribution direction (increasing or decreasing the model prediction) for all features. We note that this is subjective and context-dependent; for example, in some domains, the exact contribution values may be needed. Our prompts use a custom rubric that can be adjusted for different needs.

Completeness is scored by prompting an LLM with the explanation, explanation format, and narrative, and asking it to score completeness on a scale of 0 (missing one or more features), 1 (contains all features but missing one or more feature values or contribution directions) or 2 (includes all features, values, and contribution directions).

Again, we created a metric validation dataset of 26 human-labeled explanation-narrative pairs, as summarized in Table \ref{tab:validation-datasets}, that included narratives of different levels of completeness. We used this dataset to adjust the prompt. We started with a basic prompt (\textit{How completely does the narrative below describe the explanation given?}), but found that the LLM was regularly not noticing missing features. We addressed this by taking on a chain-of-thought \cite{wei_chain--thought_2023} approach, asking the LLM to first list out and consider whether every feature in the explanation was in the narrative before scoring.
%each with a human-labeled completeness grade of 0 (missing one or more features), 1 (includes all features but missing one or more feature values or contribution directions), or 2 (includes all features, values, and contribution directions).


We ended up with the prompt shown in Fig. \ref{fig:completeness-prompt}, which we evaluated on our metric validation dataset, scoring a total accuracy of 92\%. The full results of validation are shown in Table \ref{tab:accuracy_and_completeness}.

\subsection{Fluency}
Fluency is the degree to which the narrative sounds natural or human-written. This is highly subjective and context-dependent; therefore, for this paper we grade fluency as how closely the narrative's linguistic style matches that of a few \goldstandard{} narratives. For example, consider the following two narrative styles for the same explanation:

\textbf{Precise:} The house's size (1203 sq. ft.) increased the ML output by \$10,203. The size of the second floor (0 sq. ft.) decreased the ML output by \$4,782.

\textbf{Casual:} The house's large size increases the price prediction by about \$10,200, while its lack of a second floor decreases the prediction by about \$4,700.

Users pass in a small set of hand-written \goldstandard{} narratives (we used a set of five narratives for grading), that are then used by the \Grader{} to grade fluency. We prompted the LLM with these \goldstandard{} narratives, along with the narrative to be graded, asking it to score how well the narrative matches the style of the \goldstandard{}s on a discrete scale from 0 to 4. 

To validate our fluency scoring function, we used our nine \goldstandard{} datasets introduced in Section \ref{sec:datasets}. From each dataset, we randomly selected 5 human-written narratives as \goldstandard{}s and asked the \Grader{} LLM to compare it to the remaining human-written narratives. Table~\ref{tab:fluency-validation} shows the average fluency grades for all datasets. To validate the \Grader{}'s assessment, we confirmed whether each dataset scored highest on fluency when evaluated against \goldstandard{}s from its own data. Our original prompt, shown in Fig. \ref{fig:fluency-prompt}, did not require further adjustment, as it passed our validation.


\begin{figure}
\centering
    \prompt{
\textbf{Question:} How well does the style of the narrative match the style of these examples: 
\newline

[[\GOLDSTANDARD{} NARRATIVE 1]] 

[[\GOLDSTANDARD{} NARRATIVE 2]] 

... 

[[\GOLDSTANDARD{} NARRATIVE 5]] 
\newline 

\textbf{Narrative:} [[NARRATIVE]]
\newline

\textbf{Rubric:} 0: Very dissimilar. 1: Dissimilar. 2: Neutral. 3: Similar. 4: Very similar
\newline

\textbf{Assessment: }
}
    \caption{Prompt passed to the \Grader{} to compute the fluency metric.}
    \label{fig:fluency-prompt}
\end{figure}



% \begin{quote}
% \textbf{Question:} How well does the style of the narrative match the style of these examples: 
% \newline

% [[\GOLDSTANDARD{} NARRATIVE 1]] 

% [[\GOLDSTANDARD{} NARRATIVE 2]] 

% ... 

% [[\GOLDSTANDARD{} NARRATIVE $N$]] 
% \newline 

% \textbf{Narrative:} [[NARRATIVE]]
% \newline

% \textbf{Rubric:} 0: Very dissimilar. 1: Dissimilar. 2: Neutral. 3: Similar. 4: Very similar
% \newline

% \textbf{Assessment: }
% \end{quote}


\subsection{Conciseness}
This metric grades how long the narrative is, scaled such that shorter narratives get higher grades. We believe that, all else being equal, users will tend to prefer shorter narratives. 

This metric is computed deterministically and scaled to a continuous value between 0 and 4, using the following equation:

% \begin{equation}
% \text{score} = \max\left(0, \min\left(4, 4 \left(2 - \frac{L}{L_{\text{max}}}\right)\right)\right)
% \end{equation}

\begin{equation}
\text{grade} = 
\begin{cases} 
  0 & \text{if } L \geq 2FL_{max} \\
  4 \times \left(2 - \frac{L}{FL_{\text{max}}}\right) & \text{if } FL_{max} < L < 2FL_{max} \\
  4 & \text{if } L \leq FL_{max}
\end{cases} 
\end{equation}
 where $L$ is the number of words in the narrative, $F$ is the number of features in the input explanation, and $L_{max}$ is some configured value representing the longest ideal number of words in the narrative per feature.

In effect, this equation grades a narrative as 4 if it is shorter than some hyperparameter-defined number of words per feature, 0 if it is longer than twice this value, with grades scaling linearly between these two extremes.



% \begin{table}[]
% \caption{Average fluency grades for each dataset based on each \goldstandard{} dataset. We expect the grades down the diagonal (highlighted) to be the highest. The actual highest grades are per row are bolded. House 1/2/3: Ames Housing Dataset. Mush: Mushroom Toxicity Dataset. PDF: PDF malware dataset. Student: Student Performance Dataset.}
% \label{tab:fluency-validation}
% \begin{tabular}{@{}lcccccc@{}}
% \toprule
%                  & \multicolumn{6}{c}{\textbf{\GoldStandard{}}}                                                                                                                                                                                                    \\
%                  & \textbf{House 1}                      & \textbf{House 2}                      & \textbf{House 3}                      & \textbf{Mush}                         & \textbf{PDF}                          & \textbf{Student}                      \\ \midrule
% \textbf{House 1} & \cellcolor[HTML]{EFEFEF}\textbf{4.00} & 3.45                                  & 3.75                                  & 0.90                                  & 1.00                                  & 0.30                                  \\
% \textbf{House 2} & 3.00                                  & \cellcolor[HTML]{EFEFEF}\textbf{4.00} & 3.67                                  & 1.83                                  & 1.00                                  & 0.08                                  \\
% \textbf{House 3} & 2.31                                  & 3.38                                  & \cellcolor[HTML]{EFEFEF}\textbf{4.00} & 1.46                                  & 1.62                                  & 0.31                                  \\
% \textbf{Mush}    & 0.00                                  & 0.18                                  & 1.55                                  & \cellcolor[HTML]{EFEFEF}\textbf{4.00} & 0.64                                  & 0.91                                  \\
% \textbf{PDF}     & 0.00                                  & 0.11                                  & 2.11                                  & 3.22                                  & \cellcolor[HTML]{EFEFEF}\textbf{4.00} & 0.44                                  \\
% \textbf{Student} & 0.00                                  & 0.07                                  & 0.37                                  & 0.70                                  & 0.03                                  & \cellcolor[HTML]{EFEFEF}\textbf{3.97} \\ \bottomrule
% \end{tabular}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}


%\section{Creating the \GOLDSTANDARD{} Dataset}
%For now, we can probably create this ourselves. Our contribution in this paper is not to show that we create ``perfect'' natural-language explanations (that is too context-dependent) but rather that, given a small \goldstandard{} dataset, we can generate more explanations that fit its standards.

%After creating this \goldstandard{}, we will verify that it grades close to maximum on all metrics for all explanations. If not, we adjust the metric grading.

% \section{System}
% For evaluation and future use, we applied our work to Pyreal, a system for generating interpretable explanations. We implemented the work done in our methods section using the \texttt{NarrativeTransformer} object in this library, an object that transforms explanations into narrative formats given some hyperparameters including style samples and tuning methods.

% Our validation LLM and functions are also available through Pyreal, and used by Pyreal to optimize outputs. [or we could add this part as a separate Exlingo library]

% \begin{figure}
%     \centering
% \prompt{
% You are helping users understand an ML model's prediction. Given an explanation and information about the model, convert the explanation into a human-readable narrative.
% \newline
    
% \textbf{Example 1}
    
% \textbf{Context:} [[CONTEXT]]
    
% \textbf{Explanation:} [[EXPLANATION]]
    
% \textbf{Explanation Format:} SHAP feature contribution in (feature\_name, feature\_value, contribution) format
    
% \textbf{Narrative:} [[\GOLDSTANDARD{} NARRATIVE]]
% \newline

% \textbf{Example 2}
% \dots
    
% ---
    
% \textbf{Context:} [[CONTEXT]]

% \textbf{Explanation:} [[EXPLANATION]]

% \textbf{Explanation Format:} (feature\_name, feature\_value, SHAP\_feature\_contribution)
% \newline
    
% Please provide the output field Narrative. Do so immediately, without additional content before or after, and precisely as the format above shows.
% \newline
    
% \textbf{Narrative: }
% }
%     \caption{Prompt passed to the \Narrator{} to transform ML explanations into narratives. The \goldstandard{} narratives are taken either directly from the \goldstandard{} dataset or are bootstrapped.}
%     \label{fig:narrator-prompt}
% \end{figure}

\section{Optimizing the Narrator} \label{sec:methods}
Having validated our metric scoring functions, we sought to improve our \Narrator{} to transform explanations into narratives that optimize these metrics. Like with our \Grader{} LLM, we used DSPy programming to assemble our prompts and used the GPT-4o API for our \Narrator{} LLM\footnote{We experimented with multiple larger API-based LLM models for the \Narrator{} including GPT-3.5, GPT-4o, Claude, Gemma, and Mistral models. Based on initial results, we decided to run experiments using GPT-4o.}.
% save this for discussiona 
%For this paper, we focused on SHAP feature contribution explanations, however, our methods are fully configurable to take in diverse explanation types, through allowing configurable explanation format parameters and metric rubrics.

As shown in Figure \ref{fig:narrator-prompt-simple} we have a base prompt that instructs the LLM what it needs to do given the three inputs: the explanation, the explanation format, and the context. Below we show a few base prompts we attempted. 

%We began by following existing best practices for prompt design to develop and tune a zero-shot prompt as a baseline. We then used few-shot and bootstrapped-few shot prompting to optimize the narratives based on the metric scoring function defined in the previous section. We found that these methods were sufficient without further fine-tuning to generate accurate and complete narratives that matched the linguistic style of sample narratives. 

\textbf{Base Prompts}
We used the following prompts as a first step for baselines:

\begin{quote}
\textbf{Base Prompt 1:} You are helping users understand an ML model's prediction. Given an explanation and information about the model, convert the explanation into a human-readable narrative.
\newline

\textbf{Base Prompt 2:} You are helping users who do not have experience working with ML understand an ML model's prediction. Given an explanation and information about the model, convert the explanation into a human-readable narrative. Make your answers sound as natural as possible.
\newline

\textbf{Base Prompt 3:} You are helping users understand an ML model's prediction. Given an explanation and information about the model, convert the explanation into a human-readable narrative. Be sure to explicitly mention all values from the explanation in your response.
\end{quote}

We found that the \Narrator{} was able to generate reasonably complete and accurate narratives with these base prompts along with the the other three inputs. For the remaining experiments we only used base prompt 1, as it has the fewest tokens, scored highly on accuracy and completeness in our initial experiments, and does not include any information to suggest a specific style.

However, without examples of what a good narrative looks like for a specific application, the \Narrator{} is not able to customize the narrative style and length. For example, for an explanation from our House 1 dataset, the generated narrative using just the base prompt looks like \textit{``The model predicts the house price based on several key features. The above ground living area, which is 2090 square feet, contributes significantly to increasing the price by 16382.07 units.''} For this dataset, based on the hand-written \goldstandard{} narratives, we were seeking a narrative style more like \textit{``The relatively larger above-ground living space in this house increased its predicted price by about \$16,000.''}

As described in Section \ref{sec:datasets}, we created five hand-written narratives for each \goldstandard{} dataset. We next consider if we can add these to the prompt as examples to better customize narrative style.

%Without a style guide, however, the narratives tend to follow a generic style that is not adapted for specific use-cases. In order to provide this style guide, we turned to few-shot prompting. 
%Note: Style guide is a loaded term, it is an actual thing: https://en.wikipedia.org/wiki/Style_guide

%as prompts 2 and 3 risked coming in conflict with the desired style provided by \goldstandard{}s.
% is it human-labeled or hand-written
\textbf{Hand-Written Few-Shot.} In this experiment, we add a small number (denoted as $H$) of \goldstandard{} hand-written narratives to the prompt. These narratives were randomly selected for each prompt from the hand-written narratives we have for the \goldstandard{} dataset. 
%the same dataset used for the fluency scoring function.

%\textbf{Human-Labeled Few-Shot.} In order to better tune the narratives towards the style of the \goldstandard{} dataset, we passed a small number of \goldstandard{} sample narratives in along with the prompt. These sample narratives were randomly selected for each prompt from the \goldstandard{} dataset; the same dataset used for the fluency scoring function.

%selected is better because 
%\note{note to self: update terms}
\textbf{Bootstrapped Few-Shot.} In the previous experiment, we are limited to the hand-written narratives available to us. Additionally, these examples may not be complete, or accurate. Hence we used DSPy's \texttt{BootstrapFewShot} to create more example narratives that score highly according to our \Grader{}. To do this we give the bootstrapper
\begin{itemize}
    \item our hand-written narratives as examples;
    \item a requirement that examples it produces achieve a perfect score on accuracy, completeness, and fluency and at least 3.5 on conciseness as measured by our \Grader{}\footnote{We lowered the requirement slightly for conciseness as this significantly reduced bootstrapping time.}.
\end{itemize}

Once we have the bootstrapped examples, we add them, along with the the hand-written examples, to the prompt shown in Fig. \ref{fig:narrator-prompt-simple}. Thus the prompt now has $H$ hand-written and $B$ bootstrapped examples. With this addition, our prompt now has the base prompt, the explanation, the explanation format, the context, and $H+B$ example narratives. %An example prompt is shown in Figure~\ref{fig:narrator-prompt}. 

%\Grader{} as the metric function and the number of desired examples. 

%\begin{itemize}
 %   \item we used DSPy's \texttt{BootstrapFewShot} functionality. For this functionality, we provide XX of our hand-written narratives, it provides a set of automatically generated example B narratives.
  %  \item We then automatically score these using our \Grader{}.
   % \item Any narrative that achieved a perfect score on accuracy, completeness, and fluency and at least 3.5 on conciseness \footnote{We lowered the requirement slightly for conciseness as this significantly reduced bootstrapping time.} could be selected as a bootstrapped \goldstandard{}.
%\end{itemize} 
%Following this approach we bootstrapped 3 narratives for each application/dataset. We experimented with trying to create more than 3, but we did not get high quality narratives since we only had 5 hand-written narratives for each dataset.


%Todo question: the last sentence, who designed it and what happens if I do not say immediately and etc. this is not described as to how we arrived at this
%todo: THe algorithm for using bootstrap functionality should be described, I described from what I understood best. 
%todo: human-labeled or hand-written? Also, base prompt or Question? some clarification is required. 



%There may be significant variation in the narratives included in a \goldstandard{} dataset, and randomly selecting from this list may not lead to optimal results. Because \goldstandard{} datasets may include narratives that are not complete or accurate, a more intelligent selection and crafting of few-shot examples may improve performance. We therefore additionally experimented with bootstrapping new few-shot examples, optimized for our metric functions, using DSPy's \texttt{BootstrapFewShot} functionality. Through this process, we iteratively generated new \goldstandard{} narratives, scoring each using the \Grader{}. Any narrative that achieved a perfect score on accuracy, completeness, and fluency and at least 3.5 on conciseness\footnote{We lowered the requirement slightly for conciseness as this significantly reduced bootstrapping time.} could be selected as a \goldstandard{}.

%We experimented with prompts using different numbers of human-labeled few-shot examples (ie, those taken directly from the \goldstandard{} dataset) and bootstrapped few-shot examples. We used different combinations of $L=1, 3, 5$ and $B= 0, 1, 3, 5$, where $L=$ number of human-labeled examples from the \goldstandard{}s and $B=$ number of bootstrapped examples. 
% [note: I would not expect the bootstrap to work without any human-labeled example, how is that even possible!]
%Without at least one human-labeled example, we found that we were not able to bootstrap high-quality narratives, so we did not include conditions where $L=0$ and $B>0$. Similarly, we were not able to bootstrap large numbers of examples effectively with few labeled examples, so we did not include conditions where $L<5$ and $B=5$.

\begin{table*}
\rowcolors{1}{white}{gray!10}
\centering
\caption{Narrative quality scores for narratives generated by our \Narrator{}, as evaluated by our \Grader{}, averaged across all datasets. Metrics are reported in terms of their weighted (0-4) values. Values greater than 3.5 are in \textcolor{blue}{blue}, values less than 3 are in \textcolor{red}{red}, and the highest scoring row for each metric is in \textbf{bold}. $H$=number of hand-written few-shot examples, $B$=number of bootstrapped few-shot examples.} \label{tab:results-by-technique}
\begin{tabular}{lcccccccc}
\toprule
Base Prompt & $H$ & $B$ & Accuracy & Completeness & Fluency & Conciseness & Total grade \\
\midrule
\midrule
Base Prompt 1 & 0 & 0 & \textbf{\textcolor{blue}{4.000 $\pm$ 0.00}} & \textbf{\textcolor{blue}{4.000 $\pm$ 0.00}} & \textcolor{red}{2.467 $\pm$ 0.76} & \textcolor{red}{0.850 $\pm$ 0.94} & \textcolor{blue}{11.317 $\pm$ 1.23} \\
Base Prompt 2 & 0 & 0 & \textcolor{blue}{3.911 $\pm$ 0.27} & \textbf{\textcolor{blue}{4.000 $\pm$ 0.00}} & \textcolor{red}{2.467 $\pm$ 0.66} & \textcolor{red}{0.872 $\pm$ 0.89} & \textcolor{blue}{11.250 $\pm$ 0.97} \\
Base Prompt 3 & 0 & 0 & \textbf{\textcolor{blue}{4.000 $\pm$ 0.00}} & \textbf{\textcolor{blue}{4.000 $\pm$ 0.00}} & \textcolor{red}{2.222 $\pm$ 0.82} & \textcolor{red}{1.056 $\pm$ 1.07} & \textcolor{blue}{11.278 $\pm$ 1.44} \\
Base Prompt 1 & 1 & 0 & 3.289 $\pm$ 1.35 & \textcolor{blue}{3.511 $\pm$ 0.56} & \textcolor{blue}{3.622 $\pm$ 0.47} & \textcolor{blue}{3.749 $\pm$ 0.14} & \textcolor{blue}{14.171 $\pm$ 1.67} \\
Base Prompt 1 & 3 & 0 & 3.111 $\pm$ 1.57 & 3.422 $\pm$ 0.53 & \textcolor{blue}{3.689 $\pm$ 0.41} & \textcolor{blue}{3.708 $\pm$ 0.19} & \textcolor{blue}{13.930 $\pm$ 1.82} \\
Base Prompt 1 & 5 & 0 & 3.111 $\pm$ 1.57 & 3.289 $\pm$ 0.56 & \textcolor{blue}{3.644 $\pm$ 0.49} & \textcolor{blue}{3.669 $\pm$ 0.35} & \textcolor{blue}{13.713 $\pm$ 2.08} \\
Base Prompt 1 & 1 & 1 & \textcolor{blue}{3.800 $\pm$ 0.40} & \textcolor{blue}{3.800 $\pm$ 0.23} & \textcolor{blue}{3.650 $\pm$ 0.34} & \textcolor{blue}{3.702 $\pm$ 0.32} & \textcolor{blue}{14.952 $\pm$ 0.58} \\
Base Prompt 1 & 1 & 3 & \textcolor{blue}{3.800 $\pm$ 0.40} & \textcolor{blue}{3.800 $\pm$ 0.23} & \textcolor{blue}{3.700 $\pm$ 0.26} & \textcolor{blue}{3.734 $\pm$ 0.28} & \textbf{\textcolor{blue}{15.034 $\pm$ 0.51}} \\
Base Prompt 1 & 3 & 1 & 3.323 $\pm$ 1.34 & \textcolor{blue}{3.538 $\pm$ 0.49} & \textcolor{blue}{3.846 $\pm$ 0.19} & \textcolor{blue}{3.843 $\pm$ 0.16} & \textcolor{blue}{14.551 $\pm$ 1.72} \\
Base Prompt 1 & 3 & 3 & 3.262 $\pm$ 1.33 & \textcolor{blue}{3.631 $\pm$ 0.58} & \textcolor{blue}{3.846 $\pm$ 0.23} & \textcolor{blue}{3.890 $\pm$ 0.11} & \textcolor{blue}{14.629 $\pm$ 1.73} \\
Base Prompt 1 & 5 & 1 & 3.289 $\pm$ 1.35 & 3.333 $\pm$ 0.63 & \textbf{\textcolor{blue}{3.933 $\pm$ 0.14}} & \textcolor{blue}{3.983 $\pm$ 0.03} & \textcolor{blue}{14.538 $\pm$ 1.63} \\
Base Prompt 1 & 5 & 3 & 3.289 $\pm$ 1.35 & 3.467 $\pm$ 0.66 & \textcolor{blue}{3.889 $\pm$ 0.27} & \textbf{\textcolor{blue}{3.988 $\pm$ 0.02}} & \textcolor{blue}{14.632 $\pm$ 1.65} \\
Base Prompt 1 & 5 & 5 & 3.378 $\pm$ 1.37 & 3.422 $\pm$ 0.64 & \textcolor{blue}{3.911 $\pm$ 0.15} & \textcolor{blue}{3.977 $\pm$ 0.03} & \textcolor{blue}{14.688 $\pm$ 1.66} \\
\bottomrule

\bottomrule
\end{tabular}
\end{table*}


% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{IEEE Big Data/metrics_over_narratives.png}
%     \caption{Total number of few-shot sample narratives ($L + B$) versus each metric grade on \Narrator{}-generated narratives across all datasets.}
%     \label{fig:metrics_over_narratives}
% \end{figure}


%Our final prompt to the \Narrator{} is shown in Fig. \ref{fig:narrator-prompt}.

%Next, we discuss the quality of narratives generated with these steering approaches.
%note: steering, tuning, optimizing - pick one word through the paper!

\section{Results}

\textbf{Experimental Setup.} Using the \Narrator{} we created narratives for explanations in the \goldstandard{} datasets. We used a variety of settings for the \narrator{}: 3 prompts and 11 few-shot settings. In total, we had 169 explanations (across 9 datasets) and applied 13 techniques, resulting in 2,197 total narratives\footnote{The total LLM costs when using GPT-4o for generating and evaluating all narratives was about US\$8.44, or .38 cents per narrative to generate and evaluate on all metrics. The estimated number of inputs tokens required to transform one explanation ranges from about 150 to 1000 depending on explanation length and prompting technique.}. We scored each narrative on each of the four metrics, described in Section \ref{sec:metrics}. For the conciseness metric, we set the maximum input length to 90\% of the longest feature description from the \goldstandard{} narratives. We also used these narratives (5 per dataset) to grade fluency. The mean metric grades from our evaluation by prompting technique/few-shot setting are shown in Table \ref{tab:results-by-technique}. 

%We transformed the explanations in our evaluation datasets introduced in Section \ref{sec:datasets} into narratives using each of the prompts and few-shot settings described in Section \ref{sec:methods}. We scored each narrative on each of the four metrics, described in Section \ref{sec:metrics}. For conciseness, we set the maximum input length to 90\% of the longest feature description from the \goldstandard{} narratives. We also used these narratives (5 per dataset) to grade fluency.
\textbf{Adding examples greatly improves narrative style at a small cost to correctness.}
In Fig. \ref{fig:examples-vs-metrics}, we visualize the impact that the number of examples has on each metric. We see a clear trend of fluency and conciseness grades increasing with more examples, while accuracy and completeness grades decrease. These findings are not surprising --- without an \goldstandard{}, the \Narrator{} has nothing to match to improve fluency and conciseness. On the other hand, more examples introduces more complexity that may increase the chance of the \Narrator{} hallucinating, and increase the chance of confusing the \Narrator{} with a potentially inaccurate \goldstandard{} narrative. The fact that we see high accuracy and completeness scores without any examples demonstrates that the LLM is able to complete the task with careful prompting out-of-the-box; adding examples mainly serves to adjust the style and information included in the narrative.
 
\textbf{We see the overall highest quality narratives with a small number of hand-written and bootstrapped examples.}
Our highest total grade across all four metrics was achieved with one hand-written few-shot example and three bootstrapped examples. Having one of each style of few-shot example achieved a close second highest score.

\textbf{Bootstrapped examples contribute more to generating accurate and complete narratives.}
We also see a subtle trend in Table \ref{tab:results-by-technique} and Fig. \ref{fig:examples-vs-metrics} of bootstrapped examples improving accuracy and completeness over purely hand-written examples. This may be because bootstrapped examples must achieve perfect accuracy and completeness scores to be passed to the \Narrator{}, therefore removing the chance of passing in \goldstandard{} narratives that are either inaccurate or considered inaccurate by the \Grader{}.

%These two findings together help shed light on why balancing a small number of the two types of few-shot examples may result in the best performance.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/heatmap_metrics_tight.png}
    \caption{Correlation between mean metric grades (color) over all datasets by number of hand-written few-shot examples ($H$, x-axis) and number of bootstrapped few-shot examples ($B$, y-axis).}
    \label{fig:examples-vs-metrics}
\end{figure}

\begin{table*}
\rowcolors{1}{white}{gray!10}
\centering
\caption{Narrative quality scores generated by our \Narrator{} in our two highest-scoring conditions ($H=1, B=1,3$), averaged by dataset. Values greater than 3.5 are in \textcolor{blue}{blue}, values less than 3 are in \textcolor{red}{red}.} \label{tab:results-by-dataset}
\begin{tabular}{lcccccc}
\toprule
Dataset & Accuracy & Completeness & Fluency & Conciseness & Total score \\
\midrule
House 1 & \textcolor{blue}{3.733 $\pm$ 0.40} & \textcolor{blue}{4.000 $\pm$ 0.00} & \textcolor{blue}{3.800 $\pm$ 0.30} & \textcolor{blue}{3.719 $\pm$ 0.24} & \textcolor{blue}{15.252 $\pm$ 0.58} \\
House 2 & \textcolor{blue}{4.000 $\pm$ 0.00} & \textcolor{blue}{4.000 $\pm$ 0.00} & \textcolor{blue}{3.911 $\pm$ 0.11} & \textcolor{blue}{3.836 $\pm$ 0.16} & \textcolor{blue}{15.748 $\pm$ 0.24} \\
House 3 & \textcolor{blue}{4.000 $\pm$ 0.00} & \textcolor{blue}{3.689 $\pm$ 0.27} & \textcolor{blue}{3.933 $\pm$ 0.10} & \textcolor{blue}{3.869 $\pm$ 0.14} & \textcolor{blue}{15.491 $\pm$ 0.35} \\
Mush 1 & \textcolor{blue}{3.556 $\pm$ 0.42} & \textcolor{blue}{3.600 $\pm$ 0.00} & \textcolor{blue}{3.511 $\pm$ 0.15} & \textcolor{blue}{4.000 $\pm$ 0.00} & \textcolor{blue}{14.667 $\pm$ 0.33} \\
Mush 2 & \textcolor{red}{1.760 $\pm$ 0.88} & \textcolor{red}{2.640 $\pm$ 0.36} & \textcolor{blue}{3.920 $\pm$ 0.18} & \textcolor{blue}{3.989 $\pm$ 0.03} & \textcolor{blue}{12.309 $\pm$ 0.67} \\
PDF 1 & \textcolor{blue}{4.000 $\pm$ 0.00} & \textcolor{red}{2.400 $\pm$ 0.00} & \textcolor{blue}{4.000 $\pm$ 0.00} & \textcolor{blue}{3.977 $\pm$ 0.03} & \textcolor{blue}{14.377 $\pm$ 0.03} \\
PDF 2 & \textcolor{red}{0.000 $\pm$ 0.00} & 3.040 $\pm$ 0.22 & \textcolor{blue}{3.840 $\pm$ 0.22} & \textcolor{blue}{3.949 $\pm$ 0.02} & \textcolor{blue}{10.829 $\pm$ 0.46} \\
Student 1 & \textcolor{blue}{4.000 $\pm$ 0.00} & \textcolor{blue}{3.600 $\pm$ 0.28} & \textcolor{blue}{3.960 $\pm$ 0.09} & \textcolor{blue}{4.000 $\pm$ 0.00} & \textcolor{blue}{15.560 $\pm$ 0.36} \\
Student 2 & \textcolor{blue}{3.840 $\pm$ 0.36} & \textcolor{blue}{3.920 $\pm$ 0.18} & \textcolor{blue}{4.000 $\pm$ 0.00} & \textcolor{blue}{3.880 $\pm$ 0.15} & \textcolor{blue}{15.640 $\pm$ 0.47} \\
\bottomrule
\end{tabular}
\end{table*}


For further investigation, we report the mean metric grades by dataset for the two highest-performing few-shot settings ($H=1, B=1/3$) in Table \ref{tab:results-by-dataset}. We see unexpectedly low scores for Mush 2 and PDF datasets. Inspecting the narratives generated more closely suggests a few possible issues.

\textbf{Some narrative styles require additional information to be generated and graded.}
The low accuracy for the PDF 2 dataset may stem from the \goldstandard{} narratives for this dataset using relative terms like ``the larger file size''; the \Grader{} does not get  information about the distribution of these features, so it may be labeling these terms as inaccurate. This suggests that if narratives with such comparative words are desired, additional information should be passed in.

\textbf{Further investigation into the \Grader{} quality on diverse datasets is required.} The low scores on the Mush 2 dataset and the lower completeness score on the PDF 1 dataset appear to stem from an error with the \Grader{} rather than the \Narrator{}. For example, for the Mush 2 dataset, the narrative \textit{The lack of odor and broad gill size suggest the mushroom is more likely to be poisonous} from the explanation \textit{(odor, none, 0.15), (gill-size, broad, 0.06)} was incorrectly given a 0 on accuracy. It is possible that the LLM is ``playing it safe'', given the high-stakes application of mushroom toxicity, as a result of AI safety work (this problem may not affect Mush 1, as its narratives include safety-conscious additions like ``be careful'' or ``confirm with external sources''). However, this is speculation that requires further investigation.

In the next section, we discuss our key takeaways from these results further.


\section{Discussion and Future Work}
This work represents a first step into transforming ML explanations into narratives, and suggests several future directions. We determined that powerful modern LLMs are capable of creating high-quality narrative versions of SHAP explanations.%that match the style of a small number of hand-written and bootstrapped examples. 
Balancing hand-written and bootstrapped examples, while keeping the number of these low, appears to create the best balance between correctness (accuracy and completeness) and style (fluency and conciseness). Adding additional \goldstandard{}s can improve style at the cost of correctness (accuracy and completeness) --- users in different domains may value these metrics differently, and wish to modify the number of \goldstandard{}s accordingly. 

However, certain subtle issues --- such as including comparative terms like ``larger'' or working within complex domains --- confuse our \Grader{} into scoring narratives incorrectly. Without a highly-accurate grader, it may be difficult to generate narratives with enough trust for high-risk domains. Therefore, further investigation is needed.

\subsection{System Integration and Open-Source Implementation}
We integrated the findings from this paper in Pyreal, a library for transforming explanations for readability. We implemented the \Narrator{} in the form of the \texttt{NarrativeTransformer}
% \footnote{Instructions for transforming explanations using Pyreal can be found here: https://dtail.gitbook.io/pyreal/user-guides/using-applications-realapps/narrative-explanations-using-llms} 
object in this library, an object that transforms explanations into narratives given some hyperparameters including style samples.

Pyreal can be used to both generate the initial explanation and then transform it into narratives. Fig. \ref{fig:pyreal-code} shows a sample of the code to generate a SHAP feature contribution explanation and transform it to narrative format.

% \begin{figure}[t!]
%     \centering
%     \begin{lstlisting}[language=Python]]
%     from pyreal.transformers import (
%         NarrativeTransformer, OneHotEncoder)
%     from pyreal import RealApp
    
%     context = "The model predicts house prices"
    
%     # Explanation, narrative pairs
%     examples = {"feature_contributions": 
%             [("size, 120, -120", "The model...")]}
                    
%     narrative = NarrativeTransformer(
%                     num_features=3,
%                     context_description=context,
%                     training_examples=examples)
    
%     transformers = [OneHotEncoder(), narrative]
%     app = RealApp(model, transformers, X_train)
    
%     app.produce_feature_contributions(X)\end{lstlisting}
%     \caption{Open-source library implementation of narrative explanation generation process. The output of the final line is a dictionary with keys as row IDs in X\_train and values as narrative explanations of that model prediction on that row.}
%     \label{fig:pyreal-code}
% \end{figure}
\begin{figure}[t!]
   \centering
   \begin{lstlisting}[language=Python]]
from pyreal.transformers import NarrativeTransformer
from pyreal import RealApp
    
context = "The model predicts house prices"
    
# Explanation, narrative pairs
examples = {"feature_contributions": 
        [("size, 120, -120", "The model...")]}
                
narrative = NarrativeTransformer(
               num_features=3,
               context_description=context,
               training_examples=examples)

app = RealApp(model, transformers=[narrative])   
app.produce_feature_contributions(X, X_train)\end{lstlisting}
    \caption{Open-source library implementation of narrative generation process. The output of the final line is a dictionary with keys as row IDs in X and values as narratives of that model prediction on that row.}
    \label{fig:pyreal-code}
\end{figure}

\subsection{Lessons from Adjusting the \Grader{}}
In past work \cite{zytek_llms_2024}, we suggested that the accuracy metric be graded on a 3-point scale of \textit{inaccurate}, \textit{accurate but misleading}, or \textit{accurate}. However, discussion and experimentation revealed that ``misleading'' in this context is a highly subjective specifier, which makes it difficult for both human and LLM graders to give consistent grades. We therefore settled on a boolean 0 or 1 grade, which was sufficient for our purposes.

% We originally intended for the fluency metric to broadly describe the degree to which the narrative sounds natural or human-written, fine-tuned from a general-purpose crowd-generated \goldstandard{} dataset of narratives on a wide variety of datasets. However, we determined from discussion with diverse ML users that preferred narrative style is highly subjective and context-dependent, and therefore the fluency metric would be far more useful if based on a small, application-specific \goldstandard{} dataset.

\subsection{Future Work}
In this work we focused on SHAP contributions; however, by adjusting the input explanation format and some details in the metric rubrics, this work could easily be updated to support other kinds of explanations.

While in this paper we focus on automated grading, a natural next step would be to evaluate how effective the narratives are for real-world decision making. %This study can further validate our automated metric evaluation by correlated the automated grades with human-labeled grades. 
This study could further validate our automated metrics by correlating them with human-labeled grades.
%Another extension would be to investigate alternative automated evaluation functions, such as BLUERT \cite{sellam_bleurt_2020}.

We determined that finetuning approaches are not required to develop an effective \Narrator{} with a sufficiently powerful base LLM. However, finetuning may be beneficial to allow smaller architectures to perform the task as well as the larger models we worked with. As a first step to trying this, we applied the same final prompt (with 3 labeled few-shot examples) to a smaller, 7B parameter local model\footnote{Mistral-7B-v0.1} to determine how well it could perform one-of-the-box. The model effectively matched style, with average fluency and conciseness scores of 3.91 and 3.81, respectively. However, the small \Narrator{} did not always parse the input explanation correctly, resulting in lower accuracy and completeness scores of 0.98 and 1.64 respectively. Since smaller, local models are more practical for many real-world applications, we plan to refine prompts and explore finetuning to improve these results.

%Another future direction is to further improve the usefulness of narrative explanations by instilling them with additional context information and rationalizations. 
Another future direction is to enhance the usefulness of narrative versions of explanations by incorporating additional context and rationalizations. For example, an explanation narrative of ``This house is predicted to sell for more because it was built in the year 1930'' can be rationalized as ``In this market, older houses hold a premium because of their better building materials and unique history.'' In use cases where the model uncovered unexpected patterns in data, such rationalizations can be valuable for knowledge discovery and decision-making.

\section{Conclusion}

This work presents findings in transforming traditional ML explanations into natural-language narratives using LLMs. We developed \Explingo{}, a system for generating narrative versions of explanations. This system includes a \Narrator{} that uses LLM's to transform ML explanations into narratives, and a \Grader{} that automatically grades narratives on metrics including accuracy, completeness, fluency, and conciseness.

Our experiments show that the \Narrator{}, when properly guided by a small \goldstandard{} dataset, can generate narratives that score highly on these metrics. We found that incorporating a mix of hand-written and bootstrapped few-shot examples improves the narrative quality. 
%We additionally showed through \Grader{} validation studies that we can effectively measure the quality of narrative explanations in an automated manner. 

%Despite these advancements, our work also highlighted several challenges, including a reduction in \Grader{} quality as the domain gets more complex and explanations drift further from the \goldstandard{}s provided. These issues demonstrate the need for further refinement of our \Grader{} system, particularly for use in high-stakes decision-making environments.

This work represents a step towards enabling natural question-and-answer conversations between ML models and humans. Future research will continue this thread through  exploring additional types of explanations and conducting user studies to validate the effectiveness of narrative versions of explanations in real-world applications.
